Pruning has a disparate impact on model accuracy

Network pruning is a widely-used compression technique that is able to significantly scale down overparameterized models with minimal loss of accuracy. This paper shows that pruning may create or exacerbate disparate impacts. The paper sheds light on the factors to cause such disparities, suggesting differences in gradient norms and distance to decision boundary across groups to be responsible for this critical issue. It analyzes these factors in detail, providing both theoretical and empirical support, and proposes a simple, yet effective, solution that mitigates the disparate impacts caused by pruning.

==> NeurIPS-22_Fair-Pruning - arixv/GradientCpnt2.tex <==



\section{Why disparity in groups' gradients causes unfairness?}
\label{sec:grad_analysis}

This section analyzes the effect of gradients norms on the unfairness 
observed in the pruned models.
In more detail, it shows that unbalanced datasets result in a model with 
large differences in gradient norms between groups (Proposition 
\ref{thm:grad_imbalance}), it connects gradients norms for a group with 
the resulting model errors in such a group (Proposition 
\ref{thm:acc_vs_grad}), and connects these concepts with the excessive 
loss (Theorem \ref{thm:taylor}) 
to show that unfairness in model pruning is largely controlled by the 
difference in gradient norms among groups.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wrapfigure}[9]{r}{145pt} 
    \centering
    \vspace{-20pt}
    \includegraphics[width=\linewidth]{figures/size_vs_grad.pdf}
    \vspace{-18pt}
    \caption{\small Group size vs.~gradient norms.}
    \label{fig:size_vs_grad}
\end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{Gradient norms and group sizes.}
The section first shows that imbalanced datasets lead a model to have 
imbalanced gradient norms across groups. The following result assumes 
that the training converges to a local minima. 

\begin{proposition}
\label{thm:grad_imbalance} 
Consider two groups $a$ and $b$ in $\cA$ with $|D_a| \geq |D_b|$. Then 
\(
\left\| \bm{g}_a^\ell \right\|  \leq  \left\| \bm{g}_b^\ell \right\|.
\)
\end{proposition}
That is, groups with more data samples will result in smaller gradients 
norms than groups with fewer data samples and vice-versa. Figure \ref{fig:size_vs_grad} illustrates
Proposition \ref{thm:grad_imbalance}. The plot shows the relation between
groups sizes $|D_a|$ and their associated gradient 
norms $\|\bm{g}_a^\ell \|$ on the UTK dataset and settings described above. Notice the strong trend between decreasing group sizes and increasing gradient norms for such groups.
These theoretical considerations can be used to explain why underrepresented groups are often subject to larger performance impacts after network pruning \cite{Hooker2020CharacterisingBI}. These groups tend to exhibit large gradient norms at convergence, relative to other groups, thus, by  Theorem \ref{thm:taylor}, they are also subject to larger excessive losses due to pruning.


\paragraph{Gradient norms and accuracy.} 
Next, the section shows a strong connection between the gradient norms of a group and its associated accuracy. The following assumes the models adopt a cross entropy loss (or mean squared error for regression tasks, as shown Appendix \ref{sec:missing_proofs}). 

\begin{proposition}
\label{thm:acc_vs_grad}
For a given group $a \in \cA$, gradient norms can be upper bounded as:
\[
    \|\bm{g}_a^\ell \| \in
    \cO\left( 
    \sum_{(\bm{x}, y) \in D_a} 
    \underbrace{\|f_{\opttheta}(\bm{x}) - y \|}_{\textit{Error}}
    \times
    \left\| \nabla_{\btheta} f_{\opttheta}(\bm{x}) \right\|
    \right).
\]
\end{proposition}
The above relates gradient norms with an error measure of the classifier 
to a target label multiplied by the gradient of the predictions. 
For example, in a classification task with cross entropy loss, 
$\ell(f_{\btheta}(\bm{x}), y) = - \sum_{z \in \cY} f^z_{\btheta}
(\bm{x}) \bm{y}^z$, where $f_{\btheta}^z(\bm{x})$ represents the $z$-th element of the output associated with the soft-max 
layer of model $f_\btheta$, and $\bm{y}$ is a one-hot encoding of the true label $y$, with $\bm{y}^z$ representing its $z$-th element, then,
\begin{align*}
\hspace{-50pt}
    \| \bm{g}_a\|  
    &= \left\| \nabla_{\btheta} J(\btheta; D_a,) \right\| 
    = \left\| \nicefrac{1}{|D_a|} \sum_{(\bm{x},y) \in D_{a}} 
    \nabla_{f} \ell(f_{\btheta}(\bm{x}), y) \times 
    \nabla_{\btheta} f_{\btheta}(\bm{x}) \right\|\\
\hspace{-50pt}    
    &= \left\| \nicefrac{1}{|D_a|} \sum_{(\bm{x}, y) \in D_a} 
    (f_{\btheta}(\bm{x}) - \bm{y}) \times  
    \nabla_{\btheta} f_{\btheta}(\bm{x}) \right\|\\
\hspace{-50pt}    
    &\leq \nicefrac{1}{|D_a|}\sum_{(\bm{x}, y) \in D_a}  
    \left\| f_{\btheta}(\bm{x}) - \bm{y}  \right\| \times 
    \left\| \nabla_{\btheta} f_{\btheta}(\bm{x}) \right\|.
\end{align*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wrapfigure}[4]{r}{145pt} 
    \vspace{-80pt}
    \centering
    \includegraphics[width=\linewidth]{figures/acc_vs_grad.pdf}
    \vspace{-16pt}
    \caption{\small Accuracy vs. gradient norms.}
    \label{fig:acc_vs_norms}
\end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
A similar observation holds for mean square error loss, as illustrated 
in Appendix \ref{sec:missing_proofs}.
The observation above sheds light on the correlation between the prediction error of a group and its model gradients. 
This relation is emphasized in Figure~\ref{fig:acc_vs_norms}, which 
illustrates that the gradient norm for a given group increases as its prediction accuracy decreases.\!

Proposition \ref{thm:acc_vs_grad} allows us to link the gradient norms with the group accuracy of the resulting model, which, together with the result above will be useful to reason about the impact of gradient norms on the disparities in the group excessive losses.

\paragraph{The role of gradient norms in pruning.}
Having highlighted the connection between  gradients norms of a group 
with the accuracy of the pruned model on such a group, this section provides theoretical intuitions on the role of gradient norms in the disparate group losses during pruning. 

From Theorem \ref{thm:taylor}, notice that the excessive loss is controlled 
by term $\|\bm{g}_a^\ell \| \times \| \bartheta - \opttheta \|$. As already 
noted in Corollary \ref{cor:1}, the term $\| \bartheta - \opttheta \|$
regulates the impact of pruning on the excessive loss, as the difference between the pruned and non-pruned parameters vectors directly depends on the pruning rate. For a fixed pruning rate, however, notice that 
groups with different gradient norms will have a disparate effect on 
the resulting term. In particular, groups with very small gradients norms 
(those generally associated with highly accurate predictions) will be 
less sensitive to the effects of the pruning rate. Conversely, groups with large gradient norms will be affected by the pruning rate to a greater extent, with larger pruning rates, \emph{typically} reflecting in larger excessive losses. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering 
\begin{subfigure}[t]{0.28\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/global_pruning_accuracy_avg.pdf}
\caption{Accuracy}
\label{fig:global_pruning_accuracy_avg}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.275\textwidth}
\centering
\includegraphics[width=\textwidth]{figures/global_pruning_nonnormalizedgradnorms_avg.pdf}
\caption{Gradient Norm: $\|\bm{g}_a^\ell\|$}
\label{fig:nonnormal_GN}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.425\textwidth}
\centering
\includegraphics[width=\textwidth]
 {figures/global_pruning_nonnormalizedhessian.pdf}
\caption{Group Hessian: $\lambda(\bm{H}_a^\ell)$}
\label{fig:nonnormal_hessian}
\end{subfigure}
\caption{Accuracy, gradient norm, and group Hessian max eigenvalues of each ethnicity group, before and after increasing pruning ratios for UTK-Face dataset. The percentage of data samples across groups \textit{White, 
 Black, Asian, Indian, and Others} is $\sim 0.42, 0.19, 0.15, 0.15, 0.07$,
 respectively.}
\label{Fig:main_fig}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
These observations of the factors of disparity, accuracy, and group size,
can also be appreciated empirically in 
Figures~\ref{fig:global_pruning_accuracy_avg} and \ref{fig:nonnormal_GN}. 
The plots report accuracy (a) and gradient norms (b) on the UTKFace datasets for a variety of pruning rates. Consider group {\sl White} (containing 42\% of the total samples) and {\sl Others} (containing 7\% of the total samples). The unpruned model 
has high accuracy on the former group and small gradient norms. The accuracy of this group is insensitive to various pruning rates and even increases 
at large pruning regimes. 
In contrast, group {\sl Others} has much lower accuracy and larger 
gradient norms in the unpruned model. As the pruning rate increase, their accuracies drastically drop. As a result, in high pruning regimes, this minority group exhibits poor accuracy and very high gradient norms.

Notice that the empirical results apply to much more complex settings
than those which can be analyzed formally, thus they complement the theoretical observations.


==> NeurIPS-22_Fair-Pruning - arixv/HessianTerm2.tex <==


\section{Why disparity in groups' Hessians causes unfairness?}
\label{sec:hessian_analysis}

Having examined the properties of the groups gradients and their 
relation to unfairness in pruning, this section turns on analyzing 
how the 
Hessian associated with the loss function for a group is linked to the unfairness observed during pruning. In more detail, it connects the groups' Hessian to the distance to the decision boundary for the samples in that group and their resulting model errors (Theorem \ref{thm:hessian_norm_bound}), it illustrates a strong positive correlation between groups' Hessian and gradient norms, and links these concepts with the excessive loss (Theorem \ref{thm:taylor}) to show that unfairness in model pruning is controlled by the difference in maximum eigenvalues of the Hessians among groups.

\paragraph{Group Hessians and accuracy.}
The section first shows that groups presenting large Hessian values may suffer larger disparate impacts due to pruning, when compared with groups that have smaller Hessians. It does so by connecting the maximum eigenvalues of the groups Hessians with their distance to decision boundary and the group accuracy. The following result sheds light on these observations. It restricts its attention to models trained under binary cross entropy losses, for clarity of explanation, although an extension to a multi-class case is directly attainable. 
\begin{theorem}
\label{thm:hessian_norm_bound} 
Let $f_\theta$ be a binary classifier trained using a binary cross entropy loss. For any group $a \in \cA$, the maximum eigenvalue of the group Hessian $\lambda(\bm{H}_a^{\ell})$ can be upper bounded by:
\begin{equation}
    \lambda(\bm{H}_a^{\ell}) \leq \frac{1}{|D_a|}
    \sum_{(\bm{x}, y)\in D_a}
    \underbrace{
        \left( {f}_{\opttheta}(\bm{x}) \right) 
        \left( 1 - {f}_{\opttheta}(\bm{x}) \right)}_{\textit{Closeness to decision boundary}} 
        \times 
        \left\| \nabla_{\btheta} f_{\opttheta}(\bm {x}) \right\|^2 
     + 
         \underbrace{\left| f_{\opttheta}(\bm{x}) - y \right|}_{\textit{Error}} 
         \times 
        \lambda\left( \nabla^2_{\btheta} f_{\opttheta}(\bm{x}) \right). 
    \label{eq:hessian_norm_bound}
\end{equation}

\end{theorem}
The proof relies on derivations of the Hessian associated with model loss function and Weyl inequality. 
In other words, Theorem \ref{thm:hessian_norm_bound} highlights a direct connection between the maximum eigenvalue of the group Hessian and {\bf (1)} the closeness to the decision boundary of the group samples, and {\bf (2)} the accuracy of the group. The distance to the decision boundary is derived from \cite{cohen2019certified}. Intuitively this term is maximized when the classifier is highly uncertain about the prediction: ${f}_{\opttheta}(\bm{x}) \to 0.5$, and minimized when
it is highly certain ${f}_{\opttheta}(\bm{x}) \to 0$ or $1$, as showed in the following proposition.


\begin{proposition}
\label{prop:dist_bndry}
 Consider a binary  classifier $f_{\btheta}(\bm{x}) $. For a given sample $\bm{x} \in D $, the term ${f}_{\opttheta}(\bm{x}) (1 - {f}_{\opttheta}(\bm{x}) )$ is maximized when ${f}_{\opttheta}(\bm{x})  = 0.5$ and minimized when ${f}_{\opttheta}(\bm{x}) \in \{0,1\} $.
\end{proposition}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wrapfigure}[10]{r}{143pt} 
    \centering
    \vspace{-12pt}
    \includegraphics[width=\linewidth]{figures/H_and_acc.pdf}
    \vspace{-18pt}
    \caption{\small Group Hessians, distance to decision boundary, and~accuracy.}
    \label{fig:H_vs_acc}
\end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Observe that a group consisting of samples that are far from the decision boundary will have smaller Hessians and, thus, be less subject to a drop in accuracy due to model pruning. These results can be appreciated in Figure \ref{fig:H_vs_acc}. Notice the inverse relationship between maximum eigenvalues of the groups' Hessians and their average distance to the decision boundary. The same relation also holds for accuracy: the higher the Hessians maximum eigenvalues, the smaller the accuracy.
This is intuitive as samples which are close to the decision boundary
will be more prone to errors due to small changes in the model due 
to pruning, when compared with samples lying far from the decision boundary. 

\paragraph{Correlation between group Hessians and gradient norms.}
This section observes a positive correlation between maximum eigenvalues of the Hessian of a group and their gradient norms. This relation can be appreciated in Figure \ref{fig:H_vs_grad}. 
While mainly empirical, this observation is important as it illustrates that both the Hessian $\lambda(\bm{H}_a^\ell)$ and the gradient $\| \bm{g}_a^\ell \|$ terms appearing in the upper bound of the excessive loss $R(a)$ reported in Theorem \ref{thm:taylor} are in agreement. This relation was observed in all our experiments and settings.
Such observation allows us to infer that it is the combined 
effect of gradient norms and group Hessians that is responsible for 
the excessive loss of a group and, in turn, for the exacerbation of 
unfairness in the pruned models.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{wrapfigure}[11]{r}{130pt} 
    \centering
    \vspace{-14pt}
    \includegraphics[width=\linewidth]{figures/H_and_grads.pdf}
    \vspace{-18pt}
    \caption{\small Group Hessians and~gradient norms.}
    \label{fig:H_vs_grad}
\end{wrapfigure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\paragraph{The role of the group Hessian in pruning.}
 Having highlighted the connection between Hessian for a group with the resulting accuracy of the model on such a group, this section provides theoretical intuitions on the role of the Hessians in the disparate group losses during pruning. 

In Theorem \ref{thm:taylor}, notice that the excessive loss is controlled by term $\|\bm{H}_a^\ell \| \times \| \bartheta - \opttheta  \|^2$. 
As also noted in the previous section, the term $\| \bartheta - \opttheta  \|$
regulates the impact of pruning on the excessive loss as the difference between the pruned and non-pruned parameter vectors directly depends on the pruning rate. Similar to the observation for gradient norms, with a fixed pruning rate, groups with different Hessians will have a disparate effect on the resulting term. In particular, groups with small Hessians eigenvalues (those generally distant from the decision boundary and highly accurate) will be less sensitive to the effects of the pruning rate. Conversely, groups with large Hessians eigenvalues will be affected by the pruning rate to a greater extent, \emph{typically} resulting in larger excessive losses. 
These observations can further be appreciated empirically in Figures~\ref{fig:global_pruning_accuracy_avg} (for accuracy) and \ref{fig:nonnormal_hessian} (for maximum group Hessian eigenvalues) on the UTKFace datasets for a variety of pruning rates. 


==> NeurIPS-22_Fair-Pruning - arixv/checklist.tex <==
\section*{NeurIPS 2022 Paper Checklist}
% The NeurIPS Paper Checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. For each question in the checklist:

% You should answer yes, no, or n/a.
% You should reference the section(s) of the paper that provide support for your answer.
% You can also optionally write a short (1–2 sentence) justification of your answer.
% You are encouraged to take a look at the checklist early on as it likely will positively influence the way you do your research and write the paper, rather than treating it as an afterthought.

% Reviewers will be asked to use the checklist as one of the factors in their evaluation. The questions are mostly framed in terms of transparency: "Did you include [information]?" While "yes" is generally preferable to "no", it is perfectly acceptable to answer "no" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "no" or "n/a" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgement and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material.

\newcommand{\ans}[1]{{\color{purple}{{\em #1}}}}

\begin{enumerate}
\item For all authors
\begin{enumerate}[label=\alph*)]
	\item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
	% Claims in the paper should match theoretical and experimental results in terms of how much the results can be expected to generalize.

	% The paper's contributions should be clearly stated in the abstract and introduction, along with any important assumptions and limitations. It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.
	\ans{Yes. The paper contributions are stated in the abstract and listed in the Introduction.}

	\item (b) Have you read the ethics review guidelines and ensured that your paper conforms to them?

	\ans{Yes.}

	\item Did you discuss any potential negative societal impacts of your work?
	% Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), environmental impact (e.g., training huge models), fairness considerations (e.g., deployment of technologies that could further disadvantage historically disadvantaged groups), privacy considerations (e.g., a paper on model/data stealing), and security considerations (e.g., adversarial attacks).

	% We expect many papers to be foundational research and not tied to particular applications, let alone deployments, but being foundational does not imply that research has no societal impacts. If you see a direct path to any negative applications, you should point it out, even if it's not specific to your work. In a theoretical paper on algorithmic fairness, you might caution against overreliance on mathematical metrics for quantifying fairness and examples of ways this can go wrong. If you improve the quality of generative models, you might point out that your approach can be used to generate Deepfakes for disinformation. On the other hand, if you develop a generic algorithm for optimizing neural networks, you do not need to mention that this could enable people to train models that generate Deepfakes faster.

	% Consider different stakeholders that could be impacted by your work. It is possible that research benefits some stakeholders while harming others. Pay special attention to vulnerable or marginalized communities.

	% Consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.

	% If there are negative societal impacts, you should also discuss any mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).

	% For more information, see this unofficial guidance from last year and other resources at the broader impacts workshop at NeurIPS 2020.
	\ans{This work sheds light on the reasons behind the observed disparate impacts and fairness violations through pruning. Pruning is a widely-used compression technique for large-scale models which are deployed in settings with less resources. Thus, the insights generated by this work may have a positive societal impact.}

	\item Did you describe the limitations of your work?
	% You are encouraged to create a separate "Limitations" section in your paper.

	% Point out any strong assumptions and how robust your results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). Reflect on how these assumptions might be violated in practice and what the implications would be.

	% Reflect on the scope of your claims, e.g., if you only tested your approach on a few datasets or did a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.

	% Reflect on the factors that influence the performance of your approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be able to be reliably used to provide closed captions for online lectures because it fails to handle technical jargon.

	% We understand that authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection. It is worth keeping in mind that a worse outcome might be if reviewers discover limitations that aren't acknowledged in the paper. In general, we advise authors to use their best judgement and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
	\ans{Yes. Please, see section \ref{sec:limitations}.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
	\item Did you state the full set of assumptions of all theoretical results?
	% All assumptions should be clearly stated or referenced in the statement of any theorems.

	\ans{Yes. The assumptions were stated in or before each Theorem and also reported in the Appendix.} 

	\item Did you include complete proofs of all theoretical results?
	% The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, authors are encouraged to provide a short proof sketch to provide intuition.

	% You are encouraged to discuss the relationship between your results and related results in the literature. 

	\ans{Yes. While the main paper only contains proof sketches or intuitions, all complete proofs are reported in Appendix \ref{sec:missing_proofs}.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
	\item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
	%The instructions should contain the exact command and environment needed to run to reproduce the results.

	% Please see the NeurIPS code and data submission guidelines for more details.

	% Main experimental results include your new method and baselines. You should try to capture as many of the minor experiments in the paper as possible. If a subset of experiments are reproducible, you should state which ones are.

	% While we encourage release of code and data, we understand that this might not be possible, so "no because the code is proprietary" is an acceptable answer.

	% At submission time, to preserve anonymity, remember to release anonymized versions.
	\ans{Yes. Code, datasets and experiments were submitted in 
	the supplemental material. We also provide a  link in Appendix \ref{sec:additional_results}.}

	\item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?

	% The full details can be provided with the code, but the important details should be in the main paper.
	\ans{Yes. See Appendix  \ref{sec:additional_results}.}

	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
	% Answer "yes" if you report error bars, confidence intervals, or statistical significance tests for your main experiments.

	\ans{The main evaluation metric adopted in this work is the excessive loss (see Equations \eqref{eq:2} and \eqref{eq:3})
	which implicitly captures the randomness of the private mechanisms. Providing error bars would be misleading.}

	\item Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?

	% Ideally, you would provide the compute required for each of the individual experimental runs as well as the total compute.

	% Note that your full research project might have required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). The total compute used may be harder to characterize, but if you can do that, that would be even better.

	% You are also encouraged to use a CO2 emissions tracker and provide that information. See, for example, the experiment impact tracker (Henderson et al.), the ML CO2 impact calculator (Lacoste et al.), and CodeCarbon.

	\ans{Yes. See Appendix \ref{sec:additional_results}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
	\item If your work uses existing assets, did you cite the creators?
	% Cite the original paper that produced the code package or dataset.
	% Remember to state which version of the asset you're using.
	% If possible, include a URL.

	\ans{Yes. See References section.}

	\item Did you mention the license of the assets?

	% State the name of the license (e.g., CC-BY 4.0) for each asset.

	% If you scraped data from a particular source (e.g., website), you should state the copyright and terms of service of that source.

	% If you are releasing assets, you should include a license, copyright information, and terms of use in the package. If you are using a popular dataset, please check paperswithcode.com/datasets, which has curated licenses for some datasets. You are also encouraged to use their licensing guide to help determine the license of a dataset.

	% If you are repackaging an existing dataset, you should state the original license as well as the one for the derived asset (if it has changed).

	% If you cannot find this information online, you are encouraged to reach out to the asset's creators.
	\ans{Yes, when available.}

	\item Did you include any new assets either in the supplemental material or as a URL?

	% 	During submission time, remember to anonymize your assets. You can either create an anonymized URL or include an anonymized zip file.

	% If you cannot release (e.g., the asset contains proprietary information), state the reason.
	\ans{No new asset was required to perform this research.}

	\item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
	% 	For example, if you collected data from via crowdsourcing, did your instructions to crowdworkers explain how the data would be used?

	% Even if you used an existing dataset, you should check how data was collected and whether consent was obtained. We acknowledge this might be difficult, so please try your best; the goal is to raise awareness of possible issues that might be ingrained in our community.
	\ans{Yes. The paper uses public datasets.}

	\item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
	% There are some settings where the existence of this information is not necessarily bad (e.g., swear words occur naturally in text). This question is just to encourage discussion of potentially undesirable properties.

	% Explain how you checked this (e.g., with a script, manually on a sample, etc.).

	\ans{No. The adopted data is composed of standard benchmarks that have been used extensively in the ML literature and we believe the above does not apply.}
\end{enumerate}
	\item If you used crowdsourcing or conducted research with human subjects...

	\ans{No. This research did not use crowdsourcing.}
\end{enumerate}
% Checklist Questions

% For all authors...

% (a) Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?

% Claims in the paper should match theoretical and experimental results in terms of how much the results can be expected to generalize.

% The paper's contributions should be clearly stated in the abstract and introduction, along with any important assumptions and limitations. It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper.

% (b) Have you read the ethics review guidelines and ensured that your paper conforms to them?

% Please read the ethics review guidelines.

% (c) Did you discuss any potential negative societal impacts of your work?

% Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), environmental impact (e.g., training huge models), fairness considerations (e.g., deployment of technologies that could further disadvantage historically disadvantaged groups), privacy considerations (e.g., a paper on model/data stealing), and security considerations (e.g., adversarial attacks).

% We expect many papers to be foundational research and not tied to particular applications, let alone deployments, but being foundational does not imply that research has no societal impacts. If you see a direct path to any negative applications, you should point it out, even if it's not specific to your work. In a theoretical paper on algorithmic fairness, you might caution against overreliance on mathematical metrics for quantifying fairness and examples of ways this can go wrong. If you improve the quality of generative models, you might point out that your approach can be used to generate Deepfakes for disinformation. On the other hand, if you develop a generic algorithm for optimizing neural networks, you do not need to mention that this could enable people to train models that generate Deepfakes faster.

% Consider different stakeholders that could be impacted by your work. It is possible that research benefits some stakeholders while harming others. Pay special attention to vulnerable or marginalized communities.

% Consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.

% If there are negative societal impacts, you should also discuss any mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).

% For more information, see this unofficial guidance from last year and other resources at the broader impacts workshop at NeurIPS 2020.

% (d) Did you describe the limitations of your work?

% You are encouraged to create a separate "Limitations" section in your paper.

% Point out any strong assumptions and how robust your results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). Reflect on how these assumptions might be violated in practice and what the implications would be.

% Reflect on the scope of your claims, e.g., if you only tested your approach on a few datasets or did a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.

% Reflect on the factors that influence the performance of your approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be able to be reliably used to provide closed captions for online lectures because it fails to handle technical jargon.

% We understand that authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection. It is worth keeping in mind that a worse outcome might be if reviewers discover limitations that aren't acknowledged in the paper. In general, we advise authors to use their best judgement and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.

% If you are including theoretical results...

% (a) Did you state the full set of assumptions of all theoretical results?

% All assumptions should be clearly stated or referenced in the statement of any theorems.

% (b) Did you include complete proofs of all theoretical results?

% The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, authors are encouraged to provide a short proof sketch to provide intuition.

% You are encouraged to discuss the relationship between your results and related results in the literature. 

% If you ran experiments...

% (a) Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?

% The instructions should contain the exact command and environment needed to run to reproduce the results.

% Please see the NeurIPS code and data submission guidelines for more details.

% Main experimental results include your new method and baselines. You should try to capture as many of the minor experiments in the paper as possible. If a subset of experiments are reproducible, you should state which ones are.

% While we encourage release of code and data, we understand that this might not be possible, so "no because the code is proprietary" is an acceptable answer.

% At submission time, to preserve anonymity, remember to release anonymized versions.

% (b) Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?

% The full details can be provided with the code, but the important details should be in the main paper.

% (c) Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?

% Answer "yes" if you report error bars, confidence intervals, or statistical significance tests for your main experiments.

% (d) Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?

% Ideally, you would provide the compute required for each of the individual experimental runs as well as the total compute.

% Note that your full research project might have required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). The total compute used may be harder to characterize, but if you can do that, that would be even better.

% You are also encouraged to use a CO2 emissions tracker and provide that information. See, for example, the experiment impact tracker (Henderson et al.), the ML CO2 impact calculator (Lacoste et al.), and CodeCarbon.

% If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...

% (a) If your work uses existing assets, did you cite the creators?

% Cite the original paper that produced the code package or dataset.

% Remember to state which version of the asset you're using.

% If possible, include a URL.

% (b) Did you mention the license of the assets?

% State the name of the license (e.g., CC-BY 4.0) for each asset.

% If you scraped data from a particular source (e.g., website), you should state the copyright and terms of service of that source.

% If you are releasing assets, you should include a license, copyright information, and terms of use in the package. If you are using a popular dataset, please check paperswithcode.com/datasets, which has curated licenses for some datasets. You are also encouraged to use their licensing guide to help determine the license of a dataset.

% If you are repackaging an existing dataset, you should state the original license as well as the one for the derived asset (if it has changed).

% If you cannot find this information online, you are encouraged to reach out to the asset's creators.

% (c) Did you include any new assets either in the supplemental material or as a URL?

% During submission time, remember to anonymize your assets. You can either create an anonymized URL or include an anonymized zip file.

% If you cannot release (e.g., the asset contains proprietary information), state the reason.

% (d) Did you discuss whether and how consent was obtained from people whose data you're using/curating?

% For example, if you collected data from via crowdsourcing, did your instructions to crowdworkers explain how the data would be used?

% Even if you used an existing dataset, you should check how data was collected and whether consent was obtained. We acknowledge this might be difficult, so please try your best; the goal is to raise awareness of possible issues that might be ingrained in our community.

% (e) Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?

% There are some settings where the existence of this information is not necessarily bad (e.g., swear words occur naturally in text). This question is just to encourage discussion of potentially undesirable properties.

% Explain how you checked this (e.g., with a script, manually on a sample, etc.).

% If you used crowdsourcing or conducted research with human subjects...

% (a) Did you include the full text of instructions given to participants and screenshots, if applicable?

% Including this information in the supplemental material is fine, but if the main contribution of your paper involves human subjects, then we strongly encourage you to include as much detail as possible in the main paper.

% (b) Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?

% Examples of risks include a crowdsourcing experiment which might show offensive content or collect personal identifying information (PII). Ideally, the participants should be warned.

% Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper.  For initial submissions, do not include any information that would break anonymity, such as the institution conducting the review.

% (c) Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?

% First, provide the amount paid for each task (including any bonuses), and discuss how you determined the amount of time a task would take.

% Also include discussion on how the wage was determined and how you determined that this was a fair wage.


==> NeurIPS-22_Fair-Pruning - arixv/conclusion.tex <==



\section{Conclusion}
This work observed that pruning, while effective in compressing large models with minimal loss of accuracy, can result in substantial disparate accuracy impacts. The paper examined the factors causing such disparities both theoretically and empirically showing that: {\bf (1)} disparity in gradient norms across groups and {\bf (2)} disparity in Hessian matrices associated with the loss functions computed using a groups' data are two key factors responsible for such disparities to arise.
%%%%%%
By recognizing these factors, the paper also developed a simple yet effective retraining technique that largely mitigates the disparate impacts caused by pruning.

As reduced versions of large, overparameterized models become increasingly adopted in embedded systems to facilitate autonomous decisions, we believe that this work makes an important step toward {\em understanding} and {\em mitigating} the sources of disparate impacts observed in compressed learning models and hope it will spark awareness in this important area. 


==> NeurIPS-22_Fair-Pruning - arixv/inputs.tex <==
\usepackage{todonotes}
\usepackage{xcolor}
\usepackage{setspace}
\usepackage{multirow}
\usepackage{bm,bbm}
\usepackage{paralist}
%\usepackage{enumitem}
\newtheorem{prop}{Proposition}
\newcommand{\Lap}{\textrm{Lap}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand*{\prob}{\mathsf{P}}


\usepackage{amsmath}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{url}


%%% Comments
\newcommand{\nandoSide}[1]{\todo[caption={},color=cyan!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny FF: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\pascalSide}[1]{\todo[caption={},color=green!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny PVH: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\cuongSide}[1]{\todo[caption={},color=red!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny CT: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\nando}[1]{\todo[inline,caption={},color=cyan!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\footnotesize FF: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\cuong}[1]{\textbf{Cuong}:{\color{red}{#1}}}
\definecolor{darkgreen}{RGB}{204,102,0}

\newcommand{\JE}[1]{\todo[inline,caption={},color=blue!10!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\footnotesize JEK: #1}
\vspace{-8pt}
\end{spacing}}}

\newcommand{\JESide}[1]{\todo[caption={},color=purple!50!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny JEK: #1}
\vspace{-8pt}
\end{spacing}}}



\newcommand{\revSide}[2]{{\color{purple}{#1}}{\todo[caption={},color=purple!20!]{
\begin{spacing}{0.625}{\footnotesize #2}\end{spacing}}}}

\newcommand{\rev}[1]{{\color{purple}{#1}}
	\todo[caption={},color=purple!20!]
		{\begin{spacing}{0.625}
			{\footnotesize to review}
		\end{spacing}}
	}

\newcommand{\add}[1]{{\color{darkgreen}{#1}}}
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}
\def\aux{\mathrm{aux}}

% Math-cal
\newcommand{\cA}{\mathcal{A}} \newcommand{\cB}{\mathcal{B}} 
\newcommand{\cC}{\mathcal{C}} \newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}} \newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}} \newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}} \newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}} \newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}} \newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}} \newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}} \newcommand{\cV}{\mathcal{V}}
\newcommand{\cZ}{\mathcal{Z}} \newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}} \newcommand{\cY}{\mathcal{Y}}
\newcommand{\cW}{\mathcal{W}} \newcommand{\cX}{\mathcal{X}}

\newcommand{\EE}{\mathbb{E}} \newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}} \newcommand{\ZZ}{{\mathbb{Z}}}
\newcommand{\CC}{{\mathbb{C}}}
\newcommand{\btheta}{{\bm{\theta}}}

%%% helpers
\newcommand{\MLap}{\mathcal{M}_{\mathrm{Lap}}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}

\newcommand{\minimize}[1]{\underset{{#1}}{\text{minimize}}}
\newcommand{\maximize}[1]{\underset{{#1}}{\text{maximize}}}
% \newcommand{\st}{\text{subject to}}
\newcommand{\setcard}[1]{\scalebox{0.5}{$|#1|$}}
% \usepackage{mathtools}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\usepackage{esvect}\newcommand{\cev}[1]{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\se}[1]{\text{s}(#1)}
\newcommand{\re}[1]{\text{r}(#1)}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\smallk}{\scalebox{0.65}{$k$}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\nint}\lfloor\rceil
% make optimal notation
\makeatletter
\newcommand{\oset}[3][0ex]{\mathrel{\mathop{#3}\limits^{\vbox to#1{\kern-2\ex@\hbox{$\scriptstyle#2$}\vss}}}}
\makeatother
\newcommand{\optimal}[1]{\oset{\scalebox{.5}{$\star$}}{#1}}
\newcommand{\loss}{{\scriptstyle\Delta}}
% rescale vdots and ddots for small matrix 
\usepackage{letltxmacro}
\LetLtxMacro\orgvdots\vdots
\LetLtxMacro\orgddots\ddots


==> NeurIPS-22_Fair-Pruning - arixv/intro.tex <==


\section{Introduction}
\label{sec:intro}

As deep learning models evolve and become more powerful, they also
become larger and more costly to store and execute. The trend hinders
their deployment in resource-constrained platforms, such as embedded
systems or edge devices, which require efficient models in time and
space.  To address this challenge, studies have developed a variety
of techniques to prune the relatively insignificant or insensitive
parameters from a neural network while ensuring competitive
accuracy \cite{aghli2021combining,
baykal2019sipping,
blalock2020state,
Renda2020Comparing,
Han2015NIPS,sehwag2019compact,
zhang2018systematic}. 
When a model needs to be developed to 
fit given and certain requirements in size and resource consumption, 
a pruned model which is derived from a large, rigorously-trained, and
(often) over-parameterized model, is regarded as a de-facto standard. 
That is because it performs incomparably better than a same-size dense 
model which is trained from scratch, when the same amount of
effort and resources are invested.


In spite of its strengths, pruning has been showed to induce or 
exacerbate disparate effects in the accuracy of the resulting 
reduced models \cite{Hooker2020CharacterisingBI, Hooker2020WhatDC}. 
Intuitively, the removal of model weights affects the process 
in which the network separates different classes, which can have 
contrasting consequences for different groups of individuals.
This paper further shows that the accuracy of the pruned models tends 
to increase (decrease) more in classes that had already 
high (low) accuracy in the original model, leading to a  
``the rich get richer'' and ``the poor get poorer'' effect. 
This \emph{Matthew} effect is illustrated in Figure \ref{fig:motivation}. 
The figure shows the accuracy of a facial recognition task on 
different demographic groups for several pruning rates (indicating 
the percentage of parameters removed from the original models).
Notice how the accuracy of the majority group (White) tends to 
increase while that of the minority groups tends to decrease as the 
pruning ratio increases.

\begin{figure*}[t]
 \centering
    \includegraphics[width=\linewidth,height=100pt]{figures/motivation_UTK-ethnicity.pdf}
    \caption{Accuracy of each demographic group in the UTK-Face dataset using Resnet18 \cite{he2016deep}, at the increasing of the pruning rate.}
   \label{fig:motivation}
\end{figure*}


Following these observations, we shed light on the factors to 
cause such disparities. The theoretical findings suggest the presence 
of two key factors responsible for why accuracy disparities arise 
in pruned models: 
{\bf(1)} disparity in \emph{gradient norms} across groups, and {\bf
(2)} disparity in \emph{Hessian matrices} associated with the loss function computed using a group's data. 
Informally, the former carries information about the groups' local optimality, 
while the latter relates to model separability.
We analyze these factors in detail, providing both theoretical and
empirical support on a variety of settings, networks, and datasets. 
By recognizing these factors, we also develop a simple yet
effective training technique that largely mitigates the disparate impacts caused by pruning. The method is based on an alteration of the loss 
function to include components that penalize disparity of the average 
gradient norms and distance to decision boundary across groups. 

These findings are significant: {\em Pruning is a key enabler for
neural network models in embedded systems with deployments in
security cameras and sensors for autonomous devices for applications
where fairness is an essential need. 
Without careful consideration of the fairness impact of these
techniques, the resulting models can have profound effects on our
society and economy}. 




==> NeurIPS-22_Fair-Pruning - arixv/lib.tex <==
% Please download the latest anthology.bib from
%
% http://aclweb.org/anthology/anthology.bib.gz

@inproceedings{good:22,
  title   = {Recall Distortion in Neural Network Pruning and the Undecayed Pruning Algorithm},
  author  = {Aidan Good and Jiaqi Lin and Xin Yu and Hannah Sieg and Mikey Ferguson and Shandian Zhe and Jerzy Wieczorek and Thiago Serra},
  year    = {2022},
  booktitle = {Proceedings of the International Conference on Neural Information Processing Systems ({NeurIPS})}
}

@misc{https://doi.org/10.48550/arxiv.1412.6572,
  doi = {10.48550/ARXIV.1412.6572},
  
  url = {https://arxiv.org/abs/1412.6572},
  
  author = {Goodfellow, Ian J. and Shlens, Jonathon and Szegedy, Christian},
  
  keywords = {Machine Learning (stat.ML), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Explaining and Harnessing Adversarial Examples},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@inproceedings{guo2019sparse,
author = {Guo, Yiwen and Zhang, Chao and Zhang, Changshui and Chen, Yurong},
title = {Sparse DNNs with Improved Adversarial Robustness},
year = {2018},
booktitle = {Proceedings of the International Conference on Neural Information Processing Systems ({NeurIPS})},
pages = {240–249}
}

@article{papernot2016transferability,
  title   = {Transferability in Machine Learning: from Phenomena to Black-Box Attacks using Adversarial Samples},
  author  = {Nicolas Papernot and Patrick McDaniel and Ian Goodfellow},
  year    = {2016},
  journal = {arXiv preprint arXiv: Arxiv-1605.07277}
}

@inproceedings{NIPS2016_9d268236,
 author = {Hardt, Moritz and Price, Eric and Price, Eric and Srebro, Nati},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {D. Lee and M. Sugiyama and U. Luxburg and I. Guyon and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Equality of Opportunity in Supervised Learning},
 url = {https://proceedings.neurips.cc/paper/2016/file/9d2682367c3935defcb1f9e247a97c0d-Paper.pdf},
 volume = {29},
 year = {2016}
}

@article{barocas2017fairness,
  title={Fairness in machine learning},
  author={Barocas, Solon and Hardt, Moritz and Narayanan, Arvind},
  journal={Nips tutorial},
  volume={1},
  pages={2},
  year={2017}
}

@inproceedings{dwork2012fairness,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  pages={214--226},
  year={2012}
}


@article{mehrabi2021survey,
  title={A survey on bias and fairness in machine learning},
  author={Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--35},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{caton2020fairness,
  title={Fairness in machine learning: A survey},
  author={Caton, Simon and Haas, Christian},
  journal={arXiv preprint arXiv:2010.04053},
  year={2020}
}

@inproceedings{Fioretto:NeurIPS21b,
  title={Differentially Private Empirical Risk Minimization under the Fairness Lens},
  author={Tran, Cuong and Dinh, My and Fioretto, Ferdinando},
  booktitle={Advances in Neural Information Processing Systems},
  year={2021},
}




@article{fioretto:arxiv22b,
      title={Differential Privacy and Fairness in Decisions and Learning Tasks: A Survey}, 
      author={Ferdinando Fioretto and Cuong Tran and Pascal Van Hentenryck and Keyu Zhu},
      year={2022},
      journal={CoRR},
      volume={abs/2202.08187},
      url       = {https://arxiv.org/abs/2202.08187}
}

@inproceedings{Zhu:AAAI2021, 
title={Bias and Variance of Post-processing in Differential Privacy}, 
booktitle={Proceedings of the AAAI Conference on Artificial Intelligence}, 
author={Zhu, Keyu and Van Hentenryck, Pascal and Fioretto, Ferdinando}, 
year={2021}, 
pages={11177-11184} 
}

@inproceedings{Tran:IJCAI21,
  author    = {Cuong Tran and
               Ferdinando Fioretto and
               Pascal Van Hentenryck and
               Zhiyan Yao},
  editor    = {Zhi{-}Hua Zhou},
  title     = {Decision Making with Differential Privacy under a Fairness Lens},
  booktitle = {International Joint Conference on Artificial Intelligence {(IJCAI)}},
  pages     = {560--566},
  year      = {2021},
}

@inproceedings{Tran:AAAI21,
   author    = {Cuong Tran and
               Ferdinando Fioretto and
               Pascal Van Hentenryck},
  title     = {Differentially Private and Fair Deep Learning: {A} Lagrangian Dual
               Approach},
  booktitle = {Thirty-Fifth {AAAI} Conference on Artificial Intelligence},
  pages     = {9932--9939},
  publisher = {{AAAI} Press},
  year      = {2021},
}

%% Privacy / Fairness
@inproceedings{NEURIPS2019_eugene,
  title={Differential privacy has disparate impact on model accuracy},
  author={Bagdasaryan, Eugene and Poursaeed, Omid and Shmatikov, Vitaly},
  booktitle={Advances in Neural Information Processing Systems},
  pages={15479--15488},
  year={2019}
}

@misc{https://doi.org/10.48550/arxiv.2202.08187,
  doi = {10.48550/ARXIV.2202.08187},
  
  url = {https://arxiv.org/abs/2202.08187},
  
  author = {Fioretto, Ferdinando and Tran, Cuong and Van Hentenryck, Pascal and Zhu, Keyu},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Differential Privacy and Fairness in Decisions and Learning Tasks: A Survey},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{zhao2019inherent,
  title={Inherent tradeoffs in learning fair representations},
  author={Zhao, Han and Gordon, Geoff},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={15675--15685},
  year={2019}
}

@inproceedings{cohen2019certified,
  title={Certified adversarial robustness via randomized smoothing},
  author={Cohen, Jeremy and Rosenfeld, Elan and Kolter, Zico},
  booktitle={International Conference on Machine Learning},
  pages={1310--1320},
  year={2019},
  organization={PMLR}
}

@inproceedings{DBLP:conf/nips/TranDF21,
  author    = {Cuong Tran and
               My H. Dinh and
               Ferdinando Fioretto},
  title     = {Differentially Private Empirical Risk Minimization under the Fairness
               Lens},
  booktitle = {Advances in Neural Information Processing Systems 34},
  year      = {2021}
}


@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{keskar2016large,
  title={On large-batch training for deep learning: Generalization gap and sharp minima},
  author={Keskar, Nitish Shirish and Mudigere, Dheevatsa and Nocedal, Jorge and Smelyanskiy, Mikhail and Tang, Ping Tak Peter},
  journal={arXiv preprint arXiv:1609.04836},
  year={2016}
}



@article{zhang2019gradient,
  title={Why gradient clipping accelerates training: A theoretical justification for adaptivity},
  author={Zhang, Jingzhao and He, Tianxing and Sra, Suvrit and Jadbabaie, Ali},
  journal={arXiv preprint arXiv:1905.11881},
  year={2019}
}

@article{hwang2020fairfacegan,
  title={FairfaceGAN: Fairness-aware facial image-to-image translation},
  author={Hwang, Sunhee and Park, Sungho and Kim, Dohyung and Do, Mirae and Byun, Hyeran},
  journal={arXiv preprint arXiv:2012.00282},
  year={2020}
}


@inproceedings{houben2013detection,
  title={Detection of traffic signs in real-world images: The German Traffic Sign Detection Benchmark},
  author={Houben, Sebastian and Stallkamp, Johannes and Salmen, Jan and Schlipsing, Marc and Igel, Christian},
  booktitle={The 2013 international joint conference on neural networks (IJCNN)},
  pages={1--8},
  year={2013},
  organization={Ieee}
}
@article{blalock2020state,
  title={What is the state of neural network pruning?},
  author={Blalock, Davis and Ortiz, Jose Javier Gonzalez and Frankle, Jonathan and Guttag, John},
  journal={arXiv preprint arXiv:2003.03033},
  year={2020}
}
@article{xie2021model,
  title={Model compression via pruning and knowledge distillation for person re-identification},
  author={Xie, Haonan and Jiang, Wei and Luo, Hao and Yu, Hongyan},
  journal={Journal of Ambient Intelligence and Humanized Computing},
  volume={12},
  number={2},
  pages={2149--2161},
  year={2021},
  publisher={Springer}
}

@article{frankle2018lottery,
  title={The lottery ticket hypothesis: Finding sparse, trainable neural networks},
  author={Frankle, Jonathan and Carbin, Michael},
  journal={arXiv preprint arXiv:1803.03635},
  year={2018}
}
@misc{liang2021pruning,
      title={Pruning and Quantization for Deep Neural Network Acceleration: A Survey}, 
      author={Tailin Liang and John Glossner and Lei Wang and Shaobo Shi and Xiaotong Zhang},
      year={2021},
      eprint={2101.09671},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@misc{ye2018progressive,
      title={Progressive Weight Pruning of Deep Neural Networks using ADMM}, 
      author={Shaokai Ye and Tianyun Zhang and Kaiqi Zhang and Jiayu Li and Kaidi Xu and Yunfei Yang and Fuxun Yu and Jian Tang and Makan Fardad and Sijia Liu and Xiang Chen and Xue Lin and Yanzhi Wang},
      year={2018},
      eprint={1810.07378},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{yang2019quantization,
  title={Quantization networks},
  author={Yang, Jiwei and Shen, Xu and Xing, Jun and Tian, Xinmei and Li, Houqiang and Deng, Bing and Huang, Jianqiang and Hua, Xian-sheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7308--7316},
  year={2019}
}

@article{gou2021knowledge,
  title={Knowledge distillation: A survey},
  author={Gou, Jianping and Yu, Baosheng and Maybank, Stephen J and Tao, Dacheng},
  journal={International Journal of Computer Vision},
  volume={129},
  number={6},
  pages={1789--1819},
  year={2021},
  publisher={Springer}
}

@misc{he2015deep,
      title={Deep Residual Learning for Image Recognition}, 
      author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
      year={2015},
      eprint={1512.03385},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@inproceedings{buolamwini2018gender,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on fairness, accountability and transparency},
  pages={77--91},
  year={2018},
  organization={PMLR}
}

@article{paganini2020prune,
  title={Prune Responsibly},
  author={Paganini, Michela},
  journal={arXiv preprint arXiv:2009.09936},
  year={2020}
}



@article{augasta2013pruning,
  title={Pruning algorithms of neural networks—a comparative study},
  author={Augasta, M and Kathirvalavakumar, Thangairulappan},
  journal={Open Computer Science},
  volume={3},
  number={3},
  pages={105--115},
  year={2013},
  publisher={Versita}
}

@article{chouldechova2018frontiers,
  title={The frontiers of fairness in machine learning},
  author={Chouldechova, Alexandra and Roth, Aaron},
  journal={arXiv preprint arXiv:1810.08810},
  year={2018}
}

@inproceedings{hu2020fairnn,
  title={Fairnn-conjoint learning of fair representations for fair decisions},
  author={Hu, Tongxin and Iosifidis, Vasileios and Liao, Wentong and Zhang, Hang and Yang, Michael Ying and Ntoutsi, Eirini and Rosenhahn, Bodo},
  booktitle={International Conference on Discovery Science},
  pages={581--595},
  year={2020},
  organization={Springer}
}

@article{hosseinilearning,
  title={Learning Fair from Unfair Teachers},
  author={Hosseini, Sepidehsadat and Shabani, Mohammad Amin and Jahanara, Mohammad Mahdi and Salamatian, Bahar}
}



@article{zhu2021rich,
  title={The Rich Get Richer: Disparate Impact of Semi-Supervised Learning},
  author={Zhu, Zhaowei and Luo, Tianyi and Liu, Yang},
  journal={arXiv preprint arXiv:2110.06282},
  year={2021}
}

@misc{xu2021robust,
      title={To be Robust or to be Fair: Towards Fairness in Adversarial Training}, 
      author={Han Xu and Xiaorui Liu and Yaxin Li and Anil K. Jain and Jiliang Tang},
      year={2021},
      eprint={2010.06121},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{binns2018fairness,
  title={Fairness in machine learning: Lessons from political philosophy},
  author={Binns, Reuben},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={149--159},
  year={2018},
  organization={PMLR}
}

@misc{Census-voting-rights,
  author = {Census Bureau},
    title = {Voting Rights Determination file},
    year = {2016},
    url = {\url{https://www.census. gov/programs-surveys/decennial-census/about/voting-rights/voting-rights-determination-file.html}}
}




@inproceedings{mironov2017renyi,
  title={R{\'e}nyi differential privacy},
  author={Mironov, Ilya},
  booktitle={2017 IEEE 30th Computer Security Foundations Symposium (CSF)},
  pages={263--275},
  year={2017},
  organization={IEEE}
}

@inproceedings{berthelot2019mixmatch,
  title={Mixmatch: A holistic approach to semi-supervised learning},
  author={Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin A},
  booktitle={NIPS},
  pages={5049--5059},
  year={2019}
}

@misc{papernot:16,
    title={Semi-supervised Knowledge Transfer for Deep Learning from Private Training Data},
    author={Nicolas Papernot and Martín Abadi and Úlfar Erlingsson and Ian Goodfellow and Kunal Talwar},
    year={2016},
    eprint={1610.05755},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@misc{pichapati:19,
    title={AdaCliP: Adaptive Clipping for Private SGD},
    author={Venkatadheeraj Pichapati and Ananda Theertha Suresh and Felix X. Yu and Sashank J. Reddi and Sanjiv Kumar},
    year={2019},
    eprint={1908.07643},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{mcmahan:18,
    title={A General Approach to Adding Differential Privacy to Iterative Training Procedures},
    author={H. Brendan McMahan and Galen Andrew and Ulfar Erlingsson and Steve Chien and Ilya Mironov and Nicolas Papernot and Peter Kairouz},
    year={2018},
    eprint={1812.06210},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{alex2018frontiers,
    title={The Frontiers of Fairness in Machine Learning},
    author={Alexandra Chouldechova and Aaron Roth},
    year={2018},
    eprint={1810.08810},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}


%% Differential Privacy
@inproceedings{dwork:06,
  title={Calibrating noise to sensitivity in private data analysis},
  author={Dwork, Cynthia and McSherry, Frank and Nissim, Kobbi and Smith, Adam},
  booktitle={Proceedings of Theory of Cryptography Conference},
  pages={265--284},
  year={2006},
  organization={Springer}
}

@article{dwork:14,
  title={The algorithmic foundations of differential privacy},
  author={Dwork, Cynthia and Roth, Aaron and others},
  journal={Foundations and Trends{\textregistered} in Theoretical Computer Science},
  volume={9},
  number={3--4},
  pages={211--407},
  year={2014},
  publisher={Now Publishers, Inc.}
}

@article{soria:17,
  title={Individual differential privacy: A utility-preserving formulation of differential privacy guarantees},
  author={Soria-Comas, Jordi and Domingo-Ferrer, Josep and S{\'a}nchez, David and Meg{\'\i}as, David},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={12},
  number={6},
  pages={1418--1429},
  year={2017},
  publisher={IEEE}
}

% Empirical Privacy
@inproceedings{cormode:13,
  title={Empirical privacy and empirical utility of anonymized data},
  author={Cormode, Graham and Procopiuc, Cecilia M and Shen, Entong and Srivastava, Divesh and Yu, Ting},
  booktitle={2013 IEEE 29th International Conference on Data Engineering Workshops (ICDEW)},
  pages={77--82},
  year={2013},
  organization={IEEE}
}

@article{petti:19,
  title={Differential privacy in the 2020 US census: what will it do? Quantifying the accuracy/privacy tradeoff},
  author={Petti, Samantha and Flaxman, Abraham},
  journal={Gates Open Research},
  volume={3:1722},
  year={2020},
  publisher={Gates Foundation-Open Access}
}

@phdthesis{kassem:18,
  title={Differential Inference Testing A Practical Approach to Evaluate Anonymized Data},
  author={Kassem, Ali and Acs, Gergely and Castelluccia, Claude and Palamidessi, Catuscia},
  year={2018},
  school={INRIA}
}

@inproceedings{shokri:17,
  title={Membership inference attacks against machine learning models},
  author={Shokri, Reza and Stronati, Marco and Song, Congzheng and Shmatikov, Vitaly},
  booktitle={2017 IEEE Symposium on Security and Privacy (SP)},
  pages={3--18},
  year={2017},
  organization={IEEE}
}

%% Fairness 
@inproceedings{dwork:12,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  year={2012}
}

@inproceedings{zafar:17,
  title={Fairness beyond disparate treatment \& disparate impact: Learning classification without disparate mistreatment},
  author={Zafar, Muhammad Bilal and Valera, Isabel and Gomez Rodriguez, Manuel and Gummadi, Krishna P},
  booktitle={Proceedings of the 26th International Conference on World Wide Web (WWW)},
  year={2017}
}

@inproceedings{feldman:15,
  title={Certifying and removing disparate impact},
  author={Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  booktitle={proceedings of the 21th ACM SIGKDD international conference on knowledge discovery and data mining},
  year={2015}
}



@inproceedings{hardt:16,
 author = {Hardt, Moritz and Price, Eric and Price, Eric and Srebro, Nati},
title = {Equality of Opportunity in Supervised Learning},
booktitle = {Proceedings of Advances in Neural Information Processing Systems (NIPS)},
year = {2016}
}

@inproceedings{pujol:20,
  title={Fair decision making using privacy-protected data},
  author={Pujol, David and McKenna, Ryan and Kuppam, Satya and Hay, Michael and Machanavajjhala, Ashwin and Miklau, Gerome},
  booktitle={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency (FAT) },
  pages={189--199},
  year={2020}
}

@inproceedings{agarwal:18,
  title={A Reductions Approach to Fair Classification},
  author={Agarwal, Alekh and Beygelzimer, Alina and Dudik, Miroslav and Langford, John and Wallach, Hanna},
  booktitle = {Proceedings of the International Conference on Machine Learning ({ICML})},
  year={2018}
}

@inproceedings{fioretto2020lagrangian,
      title={Lagrangian Duality for Constrained Deep Learning}, 
      author={Ferdinando Fioretto and Pascal {Van Hentenryck} and {Terrence WK} Mak and Cuong Tran and Federico Baldo and Michele Lombardi},
      pages={118--135},
      year={2020},
      booktitle="European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases ({ECML-PKDD})"
}


@misc{Fioretto:ArXiv20b,
    title="A Lagrangian Dual Framework for Deep Neural Networks with Constraints Optimization",
    author="Ferdinando Fioretto and Terrence {W.K. Mak} and 
     Federico Baldo and Michele Lombardi and  Pascal {Van Hentenryck}",
    year="2020",
    eprint="2001.09394",
    archivePrefix="arXiv",
    primaryClass="cs.LG",
    secondaryClass="stat.ML"
}

@article{Fioretto:AAAI20, 
    title={Predicting AC Optimal Power Flows: Combining Deep Learning and Lagrangian Dual Methods}, 
    volume={34}, 
    number={01}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Fioretto, Ferdinando and Mak, {Terrence W.K.} and {Van Hentenryck}, Pascal}, 
    year={2020}, 
    pages={630-637} 
}


%% Fairness and Privacy
@inproceedings{cummings:19,
  title={On the compatibility of privacy and fairness},
  author={Cummings, Rachel and Gupta, Varun and Kimpara, Dhamma and Morgenstern, Jamie},
  booktitle={Proceedings of the Adjunct Publication of the 27th Conference on User Modeling, Adaptation and Personalization (UMAP)},
  year={2019}
}

@article{dwork35s,
  title={It’s Not Privacy and It’s Not Fair, 66 Stan},
  author={Dwork, Cynthia and Mulligan, Deirdre K},
  journal={L. Rev. Online},
  volume={35}
}

@inproceedings{ekstrand:18,
  title={Privacy for all: Ensuring fair and equitable privacy protections},
  author={Ekstrand, Michael D and Joshaghani, Rezvan and Mehrpouyan, Hoda},
  booktitle={Proceedings of  Conference on Fairness, Accountability and Transparency},
  pages={35--47},
  year={2018}
}

%% Constrained Learning
@InProceedings{Fontaine:14,
  author="Fontaine, Daniel and Laurent, Michel and {Van Hentenryck}, Pascal",
  title="Constraint-Based Lagrangian Relaxation",
  booktitle="Principles and Practice of Constraint Programming",
  year="2014",
  pages="324--339",
}



@article{Hestenes:69,
  title={Multiplier and gradient methods},
  author={Hestenes, Magnus R},
  journal={Journal of optimization theory and applications},
  volume={4},
  number={5},
  pages={303--320},
  year={1969},
  publisher={Springer}
}

@article{boyd2011distributed,
  title={Distributed optimization and statistical learning via the alternating direction method of multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan and others},
  journal={Foundations and Trends{\textregistered} in Machine learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2011},
  publisher={Now Publishers, Inc.}
}


%% Privacy / Fairness
@inproceedings{bagdasaryan:19,
  title={Differential privacy has disparate impact on model accuracy},
  author={Bagdasaryan, Eugene and Poursaeed, Omid and Shmatikov, Vitaly},
  booktitle={Proceedings of Advances in Neural Information Processing Systems (NIPS)},
  year={2019}
}

@inproceedings{goodman2016step,
  title={A step towards accountable algorithms? algorithmic discrimination and the european union general data protection},
  author={Goodman, Bryce W},
  booktitle={29th Conference on Neural Information Processing Systems (NIPS 2016), Barcelona. NIPS Foundation},
  year={2016}
}

@article{DBLP:journals/corr/SmithCST17,
  author    = {Virginia Smith and
               Chao{-}Kai Chiang and
               Maziar Sanjabi and
               Ameet Talwalkar},
  title     = {Federated Multi-Task Learning},
  journal   = {CoRR},
  volume    = {abs/1705.10467},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.10467}
}

@inproceedings{zafar2015fairness,
title={Fairness Constraints: Mechanisms for Fair Classification},
author={Muhammad Bilal Zafar and Isabel Valera and Manuel Gomez Rodriguez and Krishna P. Gummadi},
booktitle={Proceedings of Artificial Intelligence and Statistics (AISTAT)},
year={2017}
}

@inproceedings{chidlovskii2016domain,
  title={Domain adaptation in the absence of source domain data},
  author={Chidlovskii, Boris and Clinchant, St{\'e}phane and Csurka, Gabriela},
  booktitle={Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={451--460},
  year={2016},
  organization={ACM}
}

@inproceedings{xu2019achieving,
  title={Achieving Differential Privacy and Fairness in Logistic Regression},
  author={Xu, Depeng and Yuan, Shuhan and Wu, Xintao},
  booktitle={Proceedings of the 26th International Conference on World Wide Web (WWW) },
  year={2019}
}



@inproceedings{perez2017fair,
  title={Fair kernel learning},
  author={P{\'e}rez-Suay, Adri{\'a}n and Laparra, Valero and Mateo-Garc{\'\i}a, Gonzalo and Mu{\~n}oz-Mar{\'\i}, Jordi and G{\'o}mez-Chova, Luis and Camps-Valls, Gustau},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={339--355},
  year={2017},
  organization={Springer}
}

@inproceedings{kamishima2012fairness,
  title={Fairness-aware classifier with prejudice remover regularizer},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Asoh, Hideki and Sakuma, Jun},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={35--50},
  year={2012},
  organization={Springer}
}

@misc{li2019fair,
    title={Fair Resource Allocation in Federated Learning},
    author={Tian Li and Maziar Sanjabi and Virginia Smith},
    year={2019},
    eprint={1905.10497},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{liang2020think,
    title={Think Locally, Act Globally: Federated Learning with Local and Global Representations},
    author={Paul Pu Liang and Terrance Liu and Liu Ziyin and Ruslan Salakhutdinov and Louis-Philippe Morency},
    year={2020},
    eprint={2001.01523},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{kairouz2019advances,
    title={Advances and Open Problems in Federated Learning},
    author={Peter Kairouz and H. Brendan McMahan and Brendan Avent and Aurélien Bellet and Mehdi Bennis and Arjun Nitin Bhagoji and Keith Bonawitz and Zachary Charles and Graham Cormode and Rachel Cummings and Rafael G. L. D'Oliveira and Salim El Rouayheb and David Evans and Josh Gardner and Zachary Garrett and Adrià Gascón and Badih Ghazi and Phillip B. Gibbons and Marco Gruteser and Zaid Harchaoui and Chaoyang He and Lie He and Zhouyuan Huo and Ben Hutchinson and Justin Hsu and Martin Jaggi and Tara Javidi and Gauri Joshi and Mikhail Khodak and Jakub Konečný and Aleksandra Korolova and Farinaz Koushanfar and Sanmi Koyejo and Tancrède Lepoint and Yang Liu and Prateek Mittal and Mehryar Mohri and Richard Nock and Ayfer Özgür and Rasmus Pagh and Mariana Raykova and Hang Qi and Daniel Ramage and Ramesh Raskar and Dawn Song and Weikang Song and Sebastian U. Stich and Ziteng Sun and Ananda Theertha Suresh and Florian Tramèr and Praneeth Vepakomma and Jianyu Wang and Li Xiong and Zheng Xu and Qiang Yang and Felix X. Yu and Han Yu and Sen Zhao},
    year={2019},
    eprint={1912.04977},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}


@incollection{NIPS2017_6670,
title = {Recycling Privileged Learning and Distribution Matching for Fairness},
author = {Quadrianto, Novi and Sharmanska, Viktoriia},
booktitle = {NIPS},
year = {2017}
}

@misc{woodworth2017learning,
    title={Learning Non-Discriminatory Predictors},
    author={Blake Woodworth and Suriya Gunasekar and Mesrob I. Ohannessian and Nathan Srebro},
    year={2017},
    eprint={1702.06081},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}


@misc{mehrabi2019survey,
    title={A Survey on Bias and Fairness in Machine Learning},
    author={Ninareh Mehrabi and Fred Morstatter and Nripsuta Saxena and Kristina Lerman and Aram Galstyan},
    year={2019},
    eprint={1908.09635},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{article,
author = {Adel, Tameem and Valera, Isabel and Ghahramani, Zoubin and Weller, Adrian},
year = {2019},
month = {07},
pages = {2412-2420},
title = {One-Network Adversarial Fairness},
volume = {33},
journal = {Proceedings of the AAAI Conference on Artificial Intelligence},
doi = {10.1609/aaai.v33i01.33012412}
}


@article{DBLP:journals/corr/abs-1805-11202,
  author    = {Depeng Xu and
               Shuhan Yuan and
               Lu Zhang and
               Xintao Wu},
  title     = {FairGAN: Fairness-aware Generative Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1805.11202},
  year      = {2018},
  url       = {http://arxiv.org/abs/1805.11202},
  archivePrefix = {arXiv},
  eprint    = {1805.11202}
}

@incollection{zhao2019conditional,
    title={Conditional Learning of Fair Representations},
    author={Han Zhao and Amanda Coston and Tameem Adel and Geoffrey J. Gordon},
    booktitle = {ICLR},
    year={2019}
}

@article{DBLP:journals/corr/abs-1910-07162,
  author    = {Han Zhao and
               Amanda Coston and
               Tameem Adel and
               Geoffrey J. Gordon},
  title     = {Conditional Learning of Fair Representations},
  journal   = {CoRR},
  volume    = {abs/1910.07162},
  year      = {2019},
  url       = {http://arxiv.org/abs/1910.07162},
  archivePrefix = {arXiv},
  eprint    = {1910.07162},
  timestamp = {Tue, 22 Oct 2019 18:17:16 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1910-07162.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@incollection{NIPS2017_6699,
title = {Learning to Pivot with Adversarial Networks},
author = {Louppe, Gilles and Kagan, Michael and Cranmer, Kyle},
booktitle = {Advances in Neural Information Processing Systems 30},
year = {2017}
}

@incollection{NIPS2016_6374,
title = {Equality of Opportunity in Supervised Learning},
author = {Hardt, Moritz and Price, Eric and Price, Eric and Srebro, Nati},
booktitle = {NIPS},
year = {2016}
}

@inproceedings{DBLP:conf/icdm/CaldersKKAZ13,
 author    = {Toon Calders and
               Asim Karim and
               Faisal Kamiran and
               Wasif Ali and
               Xiangliang Zhang},
  title     = {Controlling Attribute Effect in Linear Regression},
  booktitle = {ICDM},
  year      = {2013}
}

@misc{edwards2015censoring,
    title={Censoring Representations with an Adversary},
    author={Harrison Edwards and Amos Storkey},
    year={2015},
    eprint={1511.05897},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{beutel2017data,
    title={Data Decisions and Theoretical Implications when Adversarially Learning Fair Representations},
    author={Alex Beutel and Jilin Chen and Zhe Zhao and Ed H. Chi},
    year={2017},
    eprint={1707.00075},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@incollection{NIPS2017_7151,
title = {On Fairness and Calibration},
author = {Pleiss, Geoff and Raghavan, Manish and Wu, Felix and Kleinberg, Jon and Weinberger, Kilian Q},
booktitle = {Advances in Neural Information Processing Systems 30},
year = {2017}
}

@inproceedings{10.5555/3327144.3327203,
author = {Donini, Michele and Oneto, Luca and Ben-David, Shai and Shawe-Taylor, John and Pontil, Massimiliano},
title = {Empirical Risk Minimization under Fairness Constraints},
year = {2018},
booktitle = {NIPS}
}


@inproceedings{Feldman2015ComputationalFP,
  title={Computational Fairness: Preventing Machine-Learned Discrimination},
  author={Michael Feldman},
  year={2015}
}

@article{DBLP:journals/corr/abs-1812-06135,
  author    = {Pranay Kr. Lohia and
               Karthikeyan Natesan Ramamurthy and
               Manish Bhide and
               Diptikalyan Saha and
               Kush R. Varshney and
               Ruchir Puri},
  title     = {Bias Mitigation Post-processing for Individual and Group Fairness},
  journal   = {CoRR},
  volume    = {abs/1812.06135},
  year      = {2018},
  url       = {http://arxiv.org/abs/1812.06135},
  archivePrefix = {arXiv},
  eprint    = {1812.06135},
  timestamp = {Tue, 01 Jan 2019 15:01:25 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1812-06135.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{10.1145/3306618.3314287,
author = {Kim, Michael P. and Ghorbani, Amirata and Zou, James},
title = {Multiaccuracy: Black-Box Post-Processing for Fairness in Classification},
year = {2019},
booktitle = {Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society}
}
  
@inproceedings{10.5555/3045118.3045244,
author = {Ganin, Yaroslav and Lempitsky, Victor},
title = {Unsupervised Domain Adaptation by Backpropagation},
year = {2015},
publisher = {JMLR.org},
booktitle = {Proceedings of the 32nd International Conference on International Conference on Machine Learning - Volume 37},
pages = {1180–1189},
numpages = {10},
location = {Lille, France},
series = {ICML’15}
}
    
@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5423-generative-adversarial-nets.pdf}
}

@inproceedings{10.1145/3306618.3314255,
author = {Oneto, Luca and Doninini, Michele and Elders, Amon and Pontil, Massimiliano},
title = {Taking Advantage of Multitask Learning for Fair Classification},
year = {2019},
booktitle = {Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society}
}

@incollection{NIPS2017_6699,
title = {Learning to Pivot with Adversarial Networks},
author = {Louppe, Gilles and Kagan, Michael and Cranmer, Kyle},
booktitle = {Advances in Neural Information Processing Systems 30},
editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
pages = {981--990},
year = {2017},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/6699-learning-to-pivot-with-adversarial-networks.pdf}
}

@article{DBLP:journals/corr/ShokriSS16,
  author    = {Reza Shokri and
               Marco Stronati and
               Vitaly Shmatikov},
  title     = {Membership Inference Attacks against Machine Learning Models},
  journal   = {CoRR},
  volume    = {abs/1610.05820},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.05820},
  archivePrefix = {arXiv},
  eprint    = {1610.05820},
  timestamp = {Mon, 13 Aug 2018 16:47:19 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ShokriSS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@article{10.1561/0400000042,
author = {Dwork, Cynthia and Roth, Aaron},
title = {The Algorithmic Foundations of Differential Privacy},
year = {2014},
issue_date = {August 2014},
publisher = {Now Publishers Inc.},
journal = {Found. Trends Theor. Comput. Sci.},
month = aug,
pages = {211–407},
numpages = {197}
}

@article{Black_2020,
   title={FlipTest},
   ISBN={9781450369367},
   url={http://dx.doi.org/10.1145/3351095.3372845},
   DOI={10.1145/3351095.3372845},
   journal={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
   publisher={ACM},
   author={Black, Emily and Yeom, Samuel and Fredrikson, Matt},
   year={2020},
   month={Jan}
}
@misc{cotter2018twoplayer,
    title={Two-Player Games for Efficient Non-Convex Constrained Optimization},
    author={Andrew Cotter and Heinrich Jiang and Karthik Sridharan},
    year={2018},
    eprint={1804.06500},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@incollection{NIPS2019_8322,
title = {Noise-tolerant fair classification},
author = {Lamy, Alex and Zhong, Ziyuan and Menon, Aditya K and Verma, Nakul},
booktitle = {NIPS},
year = {2019},
}


@InProceedings{Jagielski:20,
  title = 	 {Differentially Private Fair Learning},
  author = 	 {Jagielski, Matthew and Kearns, Michael and Mao, Jieming and Oprea, Alina and Roth, Aaron and -Malvajerdi, Saeed Sharifi and Ullman, Jonathan},
  booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning (ICML)},
  year = 	 {2019}
}

@misc{eban2016scalable,
    title={Scalable Learning of Non-Decomposable Objectives},
    author={Elad ET. Eban and Mariano Schain and Alan Mackey and Ariel Gordon and Rif A. Saurous and Gal Elidan},
    year={2016},
    eprint={1608.04802},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}


@InProceedings{pmlr-v98-cotter19a,
  title = 	 {Two-Player Games for Efficient Non-Convex Constrained Optimization},
  author = 	 {Cotter, Andrew and Jiang, Heinrich and Sridharan, Karthik},
  booktitle = 	 {Proceedings of the 30th International Conference on Algorithmic Learning Theory},
  year = 	 {2019},
  series = 	 {Proceedings of Machine Learning Research},}
}

@misc{cotter2018optimization,
    title={Optimization with Non-Differentiable Constraints with Applications to Fairness, Recall, Churn, and Other Goals},
    author={Andrew Cotter and Heinrich Jiang and Serena Wang and Taman Narayan and Maya Gupta and Seungil You and Karthik Sridharan},
    year={2018},
    archivePrefix={arXiv},
}


@misc{wang2020robust,
    title={Robust Optimization for Fairness with Noisy Protected Groups},
    author={Serena Wang and Wenshuo Guo and Harikrishna Narasimhan and Andrew Cotter and Maya Gupta and Michael I. Jordan},
    year={2020},
    archivePrefix={arXiv}
}

@misc{awasthi2019equalized,
    title={Equalized odds postprocessing under imperfect group information},
    author={Pranjal Awasthi and Matthäus Kleindessner and Jamie Morgenstern},
    year={2019},
    booktitle ={arXiv},
    primaryClass={stat.ML}
}

@InProceedings{pmlr-v80-kilbertus18a,
  title = 	 {Blind Justice: Fairness with Encrypted Sensitive Attributes},
  author = 	 {Kilbertus, Niki and Gascon, Adria and Kusner, Matt and Veale, Michael and Gummadi, Krishna and Weller, Adrian},
  year = 	 {2018},
  series = 	 {Proceedings of Machine Learning Research},
}

@misc{alabi2019cost,
    title={The Cost of a Reductions Approach to Private Fair Optimization},
    author={Daniel Alabi},
    year={2019},
    archivePrefix={arXiv},
}


@InProceedings{mozannar2020fair,
  title = 	 {Fair Learning with Private Demographic Data},
  author = 	 {Hussein Mozannar and Mesrob I. Ohannessian and Nathan Srebro},
 booktitle = {Proceedings of the International Conference on Machine Learning (ICML)},
  year = {2020}
}

@incollection{NIPS2014_5392,
title = {Extremal Mechanisms for Local Differential Privacy},
author = {Kairouz, Peter and Oh, Sewoong and Viswanath, Pramod},
booktitle = {Proceedings of Advances in Neural Information Processing Systems (NIPS)},
year = {2014}
}




@inproceedings{abadi:16,
author = {Abadi, Martin and Chu, Andy and Goodfellow, Ian and McMahan, H. Brendan and Mironov, Ilya and Talwar, Kunal and Zhang, Li},
title = {Deep Learning with Differential Privacy},
year = {2016},
booktitle = {Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security}
}


@misc{kuppam2019fair,
    title={Fair Decision Making using Privacy-Protected Data},
    author={Satya Kuppam and Ryan Mckenna and David Pujol and Michael Hay and Ashwin Machanavajjhala and Gerome Miklau},
    year={2019},
    archivePrefix={arXiv}
}


@article{JMLR:v12:chaudhuri11a,
  author  = {Kamalika Chaudhuri and Claire Monteleoni and Anand D. Sarwate},
  title   = {Differentially Private Empirical Risk Minimization},
  journal = {Journal of Machine Learning Research},
  year    = {2011},
}

@misc{shokri2016membership,
    title={Membership Inference Attacks against Machine Learning Models},
    author={Reza Shokri and Marco Stronati and Congzheng Song and Vitaly Shmatikov},
    year={2016},
    eprint={1610.05820},
    archivePrefix={arXiv},
    primaryClass={cs.CR}
}

@misc{ferdin2020lagrangian,
    title={Lagrangian Duality for Constrained Deep Learning},
    author={Ferdinando Fioretto and Pascal Van Hentenryck and Terrence WK Mak and Cuong Tran and Federico Baldo and Michele Lombardi},
    year={2020},
    eprint={2001.09394},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@InProceedings{pmlr-v97-amin19a,
  title = 	 {Bounding User Contributions: A Bias-Variance Trade-off in Differential Privacy},
  author = 	 {Amin, Kareem and Kulesza, Alex and Munoz, Andres and Vassilvtiskii, Sergei},
  booktitle = 	 {ICML},
  year = 	 {2019},
}

@article{acs2018differentially,
  title={Differentially private mixture of generative neural networks},
  author={Acs, Gergely and Melis, Luca and Castelluccia, Claude and De Cristofaro, Emiliano},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2018},
}







@article{xie2018differentially,
  title={Differentially private generative adversarial network},
  author={Xie, Liyang and Lin, Kaixiang and Wang, Shu and Wang, Fei and Zhou, Jiayu},
  journal={arXiv preprint arXiv:1802.06739},
  year={2018}
}

@article{Tran2020DifferentiallyPA,
  title={Differentially Private and Fair Deep Learning: A Lagrangian Dual Approach},
  author={Cuong Tran and Ferdinando Fioretto and Pascal {Van Hentenryck}},
  journal={ArXiv},
  year={2020},
  volume={abs/2009.12562}
}



@article{mironov2019r,
  title={R$\backslash$'enyi Differential Privacy of the Sampled Gaussian Mechanism},
  author={Mironov, Ilya and Talwar, Kunal and Zhang, Li},
  journal={ArXiv},
  year={2019},
  volume={abs/1908.10530}
}

@article{subramani2020enabling,
      title={Enabling Fast Differentially Private SGD via Just-in-Time Compilation and Vectorization}, 
      author={Pranav Subramani and Nicholas Vadivelu and Gautam Kamath},
        journal={ArXiv},
      year={2020},
     volume={abs/2010.09063}
}


@INPROCEEDINGS{Han2015NIPS,
  author={S. Han, J. Pool, J. Tran and W. J. Dally},
  booktitle={NIPS}, 
  title={Learning both weights and connections for efficient neural networks}, 
  year={2015},
  volume={},
  number={},
  url = {https://arxiv.org/abs/1506.02626v3},
}

@inproceedings{wu2016quantized,
  title={Quantized convolutional neural networks for mobile devices},
  author={Wu, Jiaxiang and Leng, Cong and Wang, Yuhang and Hu, Qinghao and Cheng, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4820--4828},
  year={2016}
}

@inproceedings{NIPS1988_07e1cd7d,
author = {Mozer, Michael C and Smolensky, Paul},
booktitle = {Advances in Neural Information Processing Systems},
editor = {D. Touretzky},
pages = {},
publisher = {Morgan-Kaufmann},
title = {Skeletonization: A Technique for Trimming the Fat from a Network via Relevance Assessment},
url = {https://proceedings.neurips.cc/paper/1988/file/07e1cd7dca89a1678042477183b7ac3f-Paper.pdf},
volume = {1},
year = {1988}
}


@inproceedings{
Renda2020Comparing,
title={Comparing Rewinding and Fine-tuning in Neural Network Pruning},
author={Alex Renda and Jonathan Frankle and Michael Carbin},
booktitle={International Conference on Learning Representations},
year={2020},
url={https://openreview.net/forum?id=S1gSj0NKvB}
}


@article{baykal2019sipping,
  title={Sipping neural networks: Sensitivity-informed provable pruning of neural networks},
  author={Baykal, Cenk and Liebenwein, Lucas and Gilitschenski, Igor and Feldman, Dan and Rus, Daniela},
  journal={arXiv preprint arXiv:1910.05422},
  year={2019}
}


@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff and others},
  journal={arXiv preprint arXiv:1503.02531},
  volume={2},
  number={7},
  year={2015}
}

@inproceedings{zhang2018systematic,
  title={A systematic dnn weight pruning framework using alternating direction method of multipliers},
  author={Zhang, Tianyun and Ye, Shaokai and Zhang, Kaiqi and Tang, Jian and Wen, Wujie and Fardad, Makan and Wang, Yanzhi},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={184--199},
  year={2018}
}



@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}



@inproceedings{luo2017thinet,
  title={Thinet: A filter level pruning method for deep neural network compression},
  author={Luo, Jian-Hao and Wu, Jianxin and Lin, Weiyao},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5058--5066},
  year={2017}
}


@article{sehwag2019compact,
      title={Towards Compact and Robust Deep Neural Networks}, 
      Author={Sehwag,Vikash  and Wang, Shiqi  and Mittal, Prateek  and Jana,Suman },
      year={2019},
      eprint={1906.06110},
      journal={preprint arXiv:1906.06110},
      primaryClass={cs.LG}
}

@inproceedings{aghli2021combining,
  title={Combining Weight Pruning and Knowledge Distillation for CNN Compression},
  author={Aghli, Nima and Ribeiro, Eraldo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3191--3198},
  year={2021}
}
@article{prakosa2021improving,
  title={Improving the accuracy of pruned network using knowledge distillation},
  author={Prakosa, Setya Widyawan and Leu, Jenq-Shiou and Chen, Zhao-Hong},
  journal={Pattern Analysis and Applications},
  volume={24},
  number={2},
  pages={819--830},
  year={2021},
  publisher={Springer}
}

@inproceedings{zhu2017prune,
  author    = {Michael Zhu and
               Suyog Gupta},
  title     = {To Prune, or Not to Prune: Exploring the Efficacy of Pruning for Model
               Compression},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Workshop Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  url       = {https://openreview.net/forum?id=Sy1iIDkPM},
  timestamp = {Thu, 04 Apr 2019 13:20:09 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/ZhuG18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{li2016pruning,
  title={Pruning filters for efficient convnets},
  author={Li, Hao and Kadav, Asim and Durdanovic, Igor and Samet, Hanan and Graf, Hans Peter},
  booktitle={Proceedings of the 5th International Conference on Learning Representations (ICLR’17)},
  year={2017}
}

@article{cifar10,
title= {CIFAR-10 (Canadian Institute for Advanced Research)},
journal= {},
author= {Alex Krizhevsky and Vinod Nair and Geoffrey Hinton},
year= {},
url= {http://www.cs.toronto.edu/~kriz/cifar.html},
abstract= {The CIFAR-10 dataset consists of 60000 32x32 colour images in 10 classes, with 6000 images per class. There are 50000 training images and 10000 test images. 

The dataset is divided into five training batches and one test batch, each with 10000 images. The test batch contains exactly 1000 randomly-selected images from each class. The training batches contain the remaining images in random order, but some training batches may contain more images from one class than another. Between them, the training batches contain exactly 5000 images from each class. },
keywords= {Dataset},
terms= {}
}


@inproceedings{he2017channel,
  title={Channel pruning for accelerating very deep neural networks},
  author={He, Yihui and Zhang, Xiangyu and Sun, Jian},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1389--1397},
  year={2017}
}


@inproceedings{
liu2018rethinking,
title={Rethinking the Value of Network Pruning},
author={Zhuang Liu and Mingjie Sun and Tinghui Zhou and Gao Huang and Trevor Darrell},
booktitle={International Conference on Learning Representations},
year={2019},
}

@inproceedings{Netzer2011ReadingDI,
  title={Reading Digits in Natural Images with Unsupervised Feature Learning},
  author={Yuval Netzer and Tao Wang and Adam Coates and A. Bissacco and Bo Wu and A. Ng},
  year={2011}
}

@inproceedings{zhifei2017cvpr,
  title={Age Progression/Regression by Conditional Adversarial Autoencoder},
  author={Zhang, Zhifei and Song, Yang and Qi, Hairong},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  organization={IEEE}
}

@inproceedings{liu2015faceattributes,
  title = {Deep Learning Face Attributes in the Wild},
  author = {Liu, Ziwei and Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
  booktitle = {Proceedings of International Conference on Computer Vision (ICCV)},
  month = {December},
  year = {2015} 
}

@MISC{JigsawURL,
howpublished={\url{https://www.kaggle.com/c/jigsaw-unintended-bias-in-toxicity-classification}}
}

@article{paszke2017automatic,
  title={Automatic differentiation in PyTorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  year={2017}
}

@article{Uniyal2021DPSGDVP,
  title={DP-SGD vs PATE: Which Has Less Disparate Impact on Model Accuracy?},
  author={Archit Uniyal and Rakshit Naidu and Sasikanth Kotti and Sahib Singh and Patrik Joslin Kenfack and FatemehSadat Mireshghallah and Andrew Trask},
  journal={ArXiv},
  year={2021},
  volume={abs/2106.12576}
}

@article{Hooker2020WhatDC,
  title={What Do Compressed Deep Neural Networks Forget},
  author={Sara Hooker and Aaron C. Courville and Gregory Clark and Yann Dauphin and Andrea Frome},
  journal={arXiv: Learning},
  year={2020}
}


@article{Hooker2020CharacterisingBI,
  title={Characterising Bias in Compressed Models},
  author={Sara Hooker and Nyalleng Moorosi and Gregory Clark and Samy Bengio and Emily L. Denton},
  journal={ArXiv},
  year={2020},
  volume={abs/2010.03058}
}

@inproceedings{Joseph2020GoingBC,
  title={Going Beyond Classification Accuracy Metrics in Model Compression},
  author={Vinu Joseph and Shoaib Ahmed Siddiqui and Aditya Bhaskara and Ganesh Gopalakrishnan and Saurav Muralidharan and Michael Garland and Sheraz Ahmed and Andreas R. Dengel},
  year={2020}
}


@article{Blakeney2021SimonSE,
  title={Simon Says: Evaluating and Mitigating Bias in Pruned Neural Networks with Knowledge Distillation},
  author={Cody Blakeney and Nathaniel Huish and Yan Yan and Ziliang Zong},
  journal={ArXiv},
  year={2021},
  volume={abs/2106.07849}
}

@article{Du2021WhatDC,
  title={What do Compressed Large Language Models Forget? Robustness Challenges in Model Compression},
  author={Mengnan Du and Subhabrata Mukherjee and Yu Cheng and Milad Shokouhi and Xia Hu and Ahmed Hassan Awadallah},
  journal={ArXiv},
  year={2021},
  volume={abs/2110.08419}
}

@inproceedings{xu-etal-2021-beyond,
    title = "Beyond Preserved Accuracy: Evaluating Loyalty and Robustness of {BERT} Compression",
    author = "Xu, Canwen  and
      Zhou, Wangchunshu  and
      Ge, Tao  and
      Xu, Ke  and
      McAuley, Julian  and
      Wei, Furu",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.832",
    doi = "10.18653/v1/2021.emnlp-main.832",
    pages = "10653--10659",
    abstract = "Recent studies on compression of pretrained language models (e.g., BERT) usually use preserved accuracy as the metric for evaluation. In this paper, we propose two new metrics, label loyalty and probability loyalty that measure how closely a compressed model (i.e., student) mimics the original model (i.e., teacher). We also explore the effect of compression with regard to robustness under adversarial attacks. We benchmark quantization, pruning, knowledge distillation and progressive module replacing with loyalty and robustness. By combining multiple compression techniques, we provide a practical strategy to achieve better accuracy, loyalty and robustness.",
}

@inproceedings{Ahia2021TheLD,
  title={The Low-Resource Double Bind: An Empirical Study of Pruning for Low-Resource Machine Translation},
  author={Orevaoghene Ahia and Julia Kreutzer and Sara Hooker},
  booktitle={EMNLP},
  year={2021}
}

@article{Xu2022CanMC,
  title={Can Model Compression Improve NLP Fairness},
  author={Guangxuan Xu and Qingyuan Hu},
  journal={ArXiv},
  year={2022},
  volume={abs/2201.08542}
}


@article{Stoychev2022TheEO,
  title={The Effect of Model Compression on Fairness in Facial Expression Recognition},
  author={Samuil Stoychev and Hatice Gunes},
  journal={ArXiv},
  year={2022},
  volume={abs/2201.01709}
}

@misc{Wiebke2022,
  doi = {10.48550/ARXIV.2201.07677},
  
  url = {https://arxiv.org/abs/2201.07677},
  
  author = {Toussaint, Wiebke and Mathur, Akhil and Kawsar, Fahim and Ding, Aaron Yi},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Tiny, always-on and fragile: Bias propagation through design choices in on-device machine learning workflows},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}


==> NeurIPS-22_Fair-Pruning - arixv/mitigation.tex <==


\section{Mitigation solution and evaluation}
\label{sec:mitigation}


The previous sections highlighted the presence of two key factors playing a role in the observed model accuracy disparities due to pruning: the difference in gradient norms, and the difference in Hessians losses across groups. This section first shows how to leverage these findings to provide a simple, yet effective solution to reduce the disparate impacts of pruning. Then, the section illustrates the benefits of this mitigating solution on a variety of tasks, datasets, and network architectures. 

\subsection{Mitigation solution} 
To achieve fairness, the aforementioned findings suggest to equalize the disparity associated with gradient norms $\| \bm{g}_a^\ell \|$ and Hessians
 $\lambda(\bm{H}_a^\ell)$ across different groups $a \in \cA$. For this goal, we adopt a constrained empirical risk minimization approach: 
\begin{align}
\label{eq:LD_slow}
    \minimize{\bm{\theta}}\;\; J(\bm{\theta}; D) 
    \quad
    \text{such that:}\;\; \| \bm{g}^\ell_a\| = \|\bm{g}^\ell\|, \;\;
    \lambda(\bm{H}_a^\ell) = \lambda(\bm{H}^\ell) \;\; \forall a \in \cA,
\end{align} 
where $\bm{g}^\ell = \nabla_\btheta J(\btheta; D)$ and $\bm{H}^\ell = \nabla^2_\btheta J(\btheta; D)$ refer to the gradients and Hessian associated with loss function $\ell$, respectively, and are computed using the whole dataset $D$. The approach \eqref{eq:LD_slow} is a common strategy adopted in fair learning tasks, and
the paper uses the Lagrangian Dual method of \citet{fioretto2020lagrangian} which exploits Lagrangian duality to extend the loss function with trainable and weighted regularization terms that encapsulate constraints violations (see Appendix \ref{sec:additional_results} for additional details). 

A shortcoming of this approach is, however, that requires computing the gradient norms and Hessian matrices of the group losses in each and every training iteration, rendering the process computationally unviable, especially for deep, overparametrized networks. 


To overcome this computational burden, we will use two observations made earlier in the paper. First, recall the strong relation between gradient norms for a group and their associated losses. This aspect was noted in Proposition \ref{thm:acc_vs_grad}. That is, when the losses across the groups are similar, the gradient norms across such groups will also tend to be similar. Next, Theorem \ref{thm:hessian_norm_bound} noted a positive correlation between model errors (and thus loss values) for a group and its associated Hessian eigenvalues. Thus, when the losses across the groups are similar, the group Hessians will also tend to be similar. This intuition is also complemented by the strong correlation between group Hessians and gradient norms reported in Section \ref{sec:hessian_analysis}.
%%%
Based on the above observations, we propose a simpler version of the constrained minimizer \eqref{eq:LD_slow} defined as
\begin{align}
\label{eq:LD_fast}
    \minimize{\bm{\theta}}\;\; J(\bm{\theta}; D) 
    \quad
    \text{such that:}\;\; J(\bm{\theta}; D_a) = J(\bm{\theta}; D)  
    \;\; \forall a \in \cA,
\end{align}
that substitutes the gradient norms and max eigenvalues of group Hessians equality constraints with proxy terms capturing the group $J(\btheta; D_a)$ and population $J(\btheta; D)$ losses.

\begin{wrapfigure}[17]{r}{0.5\textwidth}
\vspace{-16pt}
\centering
\includegraphics[width=\linewidth]{figures/fair_models_grad_hessian_UTK-ethnicity.pdf}
\vspace{-12pt}
\caption{Effects of fairness constraints in balancing not only group accuracy (left) but also gradient norms (middle) and group average distance to the decision boundary (right).}
\label{fig:example_mitigation}
\end{wrapfigure}
The impact of such proxy terms in the fairness-constrained problem above can be appreciated, empirically, in Figure \ref{fig:example_mitigation}. The plots, that use the UTK-Face dataset, with Ethnicity as protected group, show an original unfair model (top) and a fair counterpart obtained through problem \eqref{eq:LD_fast} (bottom). 
Both top and bottom sub-figures use an unpruned model. The top sub-figure shows the performance of an original unpruned model trained by minimizing the empirical risk function while the bottom one shows the effect of solving Problem \eqref{eq:LD_fast}, i.e., it constrains the empirical risk function with the various group loss terms. 
Notice how enforcing balance in the group losses also helps reducing and balancing the gradient norms and group's  average distance to the decision boundary. As a consequence, the resulting model fairness is dramatically enhanced (bottom-left subplot). 



\subsection{Assessment of the mitigation solution}\label{sec:AssmtMitigation}

%and \rev{CelbA} \cite{liu2015faceattributes} 
\paragraph{Datasets, models, and settings.}
This section analyzes the results obtained using the proposed mitigation solution with ResNet50 and VGG19 on the UTKFace dataset \cite{zhifei2017cvpr}, CIFAR-10~\cite{cifar10}, and SVHN~\cite{Netzer2011ReadingDI} for various protected attributes. The experiments compare the following four models:

$\bullet$ {\sl No Mitigation}: it refers to the standard pruning approach which uses no fairness mitigation strategy.\\ 
$\bullet$ {\sl Fair Bf Pruning}: it applies the fairness mitigation process (Problem \eqref{eq:LD_fast}) exclusively to the original large network, thus \emph{before} pruning.\\
$\bullet$ {\sl Fair Aft Pruning}: it applies the mitigation exclusively to the pruned network, thus \emph{after} pruning. \\
$\bullet$ {\sl Fair Both}: it applies the mitigation both to the original large network and to the pruned network.

The experiments report the overall accuracy of resulting models as well as their fairness violations, defined here as the difference between the maximal and minimal group accuracy. The reported metrics are the average of $10$ repetitions. Additional details on datasets, architectures, and hyper-parameters adopted, as well as additional and extended results are reported in Appendix \ref{sec:additional_results}.


\begin{figure*}[t]
 \centering
\includegraphics[width=0.45\linewidth]%,height=80pt]
 {figures/line_UTK_ethnicity_ResNet.pdf}
 \hspace{20pt}
\includegraphics[width=0.45\linewidth]%,height=80pt]
 {figures/line_UTK_age_bins_ResNet.pdf}
\caption{Accuracy and Fairness violations attained by all models on ResNet50, UTK-Face dataset with {\sl ethnicity} (5 classes) as group attribute (and labels) [left]  and {\sl age} (9 classes) [right].}
 \label{fig:mitigation_pruning-1}
\end{figure*}

\begin{figure*}[t]
 \centering
\includegraphics[width=0.45\linewidth]%,height=80pt]
 {figures/line_CIFAR_ResNet.pdf}
 \hspace{20pt}
\includegraphics[width=0.45\linewidth]%,height=80pt]
 {figures/line_SVHN_ResNet.pdf}
\caption{Accuracy and Fairness violations attained by all models on VGG-19, CIFAR-10 dataset (left) and SVHN (right) with 10 class labels also used as group attribute.}
 \label{fig:mitigation_pruning-2}
\end{figure*}



\paragraph{Effects on accuracy.}
The section first focuses on analyzing the effects of accuracy drop due to applying the proposed mitigation solution for fair pruning. Figure \ref{fig:mitigation_pruning-1} compares the four models on the UTK-Face dataset using a ResNet50 architecture. The left subplots use {\sl ethnicity} as protected group and class label, with $|\cY| = 5$, while the right subplots use {\sl age} as protected group and class label, with $|\cY| = 9$. Notice that, as expected, all compared models present some accuracy deterioration as the pruning rate increases. However, notably, the deterioration of the models that apply the fair mitigation steps are comparable to (or even improved) those of the "{\sl No mitigation}" model, which applies standard pruning. 

A similar trend can be seen in Figure \ref{fig:mitigation_pruning-2} that reports results on CIFAR (left) and SVHN (right). Both use the ten class labels as protected attributes. These results clearly illustrate the ability of the mitigating solution to preserve highly accurate models. 

A comparison of the ``full'' (Equation \ref{eq:LD_slow}) and ``relaxed'' (Equation \ref{eq:LD_fast}) versions of the proposed mitigation solutions is 
provided in Table~\ref{tab:full_relaxed_results}. We note that while the "full" version leads to fairer results, the reduction in the various groups accuracy is often insubstantial. We also note that the running time of the "full" version is largely (over an order magnitude) longer than the relaxed counterpart. This is due to the calculation of gradient norms and the Hessian terms associated with each group. 


\begin{table}[t]
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{@{}rr@{\hspace{10pt}}ll@{}}
\toprule
{\bf Dataset} & {\bf version} & {\bf Class-wise accuracy} & {\bf Overall accuracy} \\
  \midrule
\multirow{2}{*}{\bf UTK-age bins}   & {\bf full}    & 0.856, 0.128, 0.145, 0.319, 0.331, 0.342, 0.181, 0.334, 0.512 & 0.395 \\
                                    & {\bf relaxed} & 0.810, 0.096, 0.141, 0.284, 0.385, 0.324, 0.227, 0.257, 0.533 & 0.390 \\[0.25em]
\multirow{2}{*}{\bf UTK-gender}	    & {\bf full}    & 0.830, 0.876	& 0.857\\
                                    & {\bf relaxed} & 0.868, 0.845  & 0.852\\[0.25em]
\multirow{2}{*}{\bf SVHN}	        & {\bf full}    & 0.864, 0.911, 0.869, 0.819, 0.887, 0.784, 0.840, 0.877, 0.805, 0.856 & 0.857\\ 
                                    & {\bf relaxed} & 0.824, 0.910, 0.775, 0.726, 0.827, 0.752, 0.747, 0.789, 0.713, 0.755 & 0.795\\[0.25em]
\multirow{2}{*}{\bf MNIST}	        & {\bf full}    & 0.998, 0.996, 0.993, 0.998, 0.994, 0.991, 0.991, 0.993, 0.992, 0.985 & 0.993\\
                                    & {\bf relaxed} & 0.994, 0.988, 0.989, 0.986, 0.987, 0.979, 0.981, 0.988, 0.969, 0.994 & 0.986\\
\bottomrule
\end{tabular}%
}
\caption{Full (Equation \ref{eq:LD_slow}) vs relaxed (Equation \ref{eq:LD_fast}) versions of the proposed mitigation solutions.}
\label{tab:full_relaxed_results}
\end{table} 




\paragraph{Effects on fairness.}
The section next illustrates the ability of the proposed solution to achieve fair pruned models. 
Table \ref{tab:protected_attr_results} illustrates the results for the UTKFaces dataset with ethnicity as class labels and age as 
protected attributes for a CNN with two convolutional layers and three linear layers and prune amounts: 30\%, 50\%, 70\%, and 90\%. 
Notice how Fair Aft pruning and Fair both achieve relatively lesser fairness violations compared to the No mitigation and 
the Fair bf Pruning methods in most cases.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t]
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{@{}r@{\hspace{10pt}} l@{\hspace{5pt}}l@{\hspace{5pt}}l@{\hspace{5pt}}l @{\hspace{10pt}} l@{\hspace{5pt}}l@{\hspace{5pt}}l@{\hspace{5pt}}l@{}}
\toprule
{\bf Methods}          & \multicolumn{4}{c}{\bf Overall accuracy}           & \multicolumn{4}{c}{\bf Fairness violations} \\ 
                       & 30\% & 50\% & 70\% & 90 \% & 30\% & 50\% & 70\% & 90\%  \\
\midrule

{\bf No mitigation}    & 0.546 & 0.545 & 0.529 & 0.559 & 0.179 & 0.186 & 0.152 & 0.134 \\
{\bf Fair bf Pruning}  & 0.539 & 0.557 & 0.529 & 0.540 & 0.189 & 0.190 & 0.174 & 0.238 \\
{\bf Fair Aft Pruning} & 0.538 & 0.532 & 0.497 & 0.472 & 0.172 & 0.161 & 0.163 & 0.05  \\
{\bf Fair both}        & 0.525 & 0.541 & 0.508 & 0.484 & 0.170 & 0.144 & 0.156 & 0.073 \\ 
\bottomrule
\end{tabular}%
}
\caption{Accuracy and fairness violations for the UTKFaces dataset with \emph{ethnicity} as class labels and \emph{age} as protected attributes and prune amounts of 30\%, 50\%, 70\%, and 90\%.}
\label{tab:protected_attr_results}
\end{table}



Next, the second and fourth subplots presented in Figures \ref{fig:mitigation_pruning-1} and \ref{fig:mitigation_pruning-2} illustrate the fairness violations obtained by the four models analyzed on different datasets and settings. 
We make the following observations: First, all the plots exhibit a consistent trend in that the mitigation solution produces models which improve the fairness of the baseline, "{\sl No mitigation}" model. 
Observe that, as already illustrated in Figure \ref{fig:example_mitigation}, the fair models tend to equalize the gradient norms and group Hessians components (and thus the distance to the decision boundary across groups). Thus, the resulting pruned models also attain better fairness, when compared to their standard counterparts. 

Next, notice that "{\sl Fair Aft Pruning}" often achieves better fairness violations than "{\sl Fair Bf Pruning}", especially at high pruning regimes. This is because the former has the advantage to apply the mitigation solution directly to the pruned model to ensure that the resulting model has low differences in gradient norms and group Hessians. The presentation also illustrates the application of the mitigation strategies both before and after pruning ({\sl Fair Both}) which shows once again the significance of applying the mitigation solution over the pruned network. 

Finally, it is notable that "{\sl Fair Aft Pruning}" achieves good reductions in fairness violation. Indeed, pre-trained large (non-pruned) fair models may not be available and the ability to retrain these large models prior to pruning may be hindered by their size and complexity. 


==> NeurIPS-22_Fair-Pruning - arixv/probFormulation.tex <==


\section{Problem settings and goals}
The paper considers datasets $D$ consisting of $n$ datapoints 
$(\bm{x}_i, a_i, y_i)$, with $i \in [n]$, drawn i.i.d.~from an unknown
distribution $\Pi$. Therein, $\bm{x}_i \in \cX$ is a feature vector,
$a_i \in \cA$ with $\cA = [m]$ (for some finite $m$) is a demographic group 
attribute, and $y_i \in \cY$ is a class label. For example, consider the 
case of a face recognition task. The training example feature $\bm{x}_i$ may 
describe a headshot of an individual, the protected attribute $a_i$
may describe the individual's gender or ethnicity, and $y_i$ represents
the identity of the individual. 
The goal is to learn a predictor $f_\btheta : \cX \to \cY$, where $\btheta$
is a $k$-dimensional real-valued vector of parameters that minimizes 
the empirical risk function:
\begin{align}
\label{eq:erm}
\optimal{\btheta} = \argmin_\btheta J(\bm{\btheta}; D) = 
\frac{1}{n} \sum_{i=1}^n \ell(f_\btheta(\bm{x}_i), y_i),
\end{align}
where $\ell: \cY \times \cY \to \RR_+$ is a non-negative \emph{loss function} 
that measures the model quality. 

We focus on analyzing properties arising when extracting a small model $f_{\bar{\btheta}}$ with $\bar{\btheta} \subset\, \optimal{\btheta}$ of size $|\bar{\btheta}| = \bar{k} \ll k$.
Model $f_{\bar{\btheta}}$ is constructed by pruning the least important 
values or filters from vector $\optimal{\btheta}$ (i.e., those with smaller 
values in magnitude) according to a prescribed criterion, such as an $\ell_p$ 
norm \cite{NIPS1988_07e1cd7d, Han2015NIPS}.
The paper focuses on understanding the fairness impacts (as defined next) 
arising when pruning general classifiers, such as neural networks. 

\paragraph{Fairness}
The fairness analysis focuses on the notion of \emph{excessive loss}, 
defined as the difference between the original and the pruned risk 
functions over some group $a \in \cA$:
\begin{equation}
\label{eq:2}
    R(a) = J(\bar{\btheta}; D_a) - J(\optimal{\btheta}; D_a),
\end{equation}
where $D_a$ denotes the subset of the dataset $D$ containing samples 
($\bm{x}_i, a_i, y_i$) whose group membership $a_i = a$. 
Intuitively, the excessive loss represents the change in loss (and thus, in 
accuracy) that a given group experiences as a result of pruning.
Fairness is measured in terms of the maximal \emph{excessive loss difference}, 
also referred to as \emph{fairness violation}:
\begin{equation}
\label{eq:3}
    \xi(D) = \max_{a, a' \in \cA} |R(a) - R(a')|,
\end{equation}
defining the largest excessive loss difference across all protected groups. 
(Pure) fairness is achieved when $\xi(D) = 0$, and thus 
a fair pruning method aims at minimizing the excessive loss difference. 

The goal of this paper is to shed light on why fairness issues arise 
(i.e., $ R(a) > 0)$ as a result of pruning, why some groups suffer more than others (i.e., $R(a) > R(a'))$, and what mitigation measures could be taken
to minimize unfairness due to pruning.

We use the following notation: variables are denoted by calligraph 
symbols, vectors or matrices by bold symbols, and sets by uppercase symbols. 
Finally, $\| \cdot \|$ denotes the Euclidean norm and we use
$f_{\btheta}(\bm{x})$ to refer to the model' \emph{soft} outputs.
All proofs are reported in Appendix~\ref{sec:missing_proofs}.

\iffalse
To encourage accuracy parity fairness of the classifier, we can add the following equality constraints to the objective function in Equation \ref{eq:erm}.

\begin{equation}
   J(\mathcal{D}_a, \btheta) = J(\mathcal{D}, \btheta) \, \forall a \in \cA
\end{equation}

The above fairness constraint requires the average classification loss per group $a$ is similar with that's at population level. To learn the fair classifier $\btheta_f$ under such fairness constraint, we can employ the Dual Lagrangian framework \cite{fioretto2020lagrangian}. First, the Lagrangian loss of the fair problem can be written as follows:

\begin{equation}
    \cL(\theta, \lambda, \cD) = J(\cD, \theta) + \sum_{a \in \cA} \lambda_a | J(\cD, \theta) - J(\cD, \theta),
\end{equation}
where $\lambda_a \geq 0, \forall a \in \cA$ are the multipliers. The training process consists of primal and dual update steps. 

In the primal update steps, we are updating the classifiers' parameters $\theta$ given fixed multipliers $\lambda$.


\begin{equation}
  \theta^*(\lambda) = \mbox{argmin}_{\theta} \cL(\theta, \lambda, \cD)
\end{equation}

In the dual update steps, we are updating the multipliers $\lambda$ given fixed model parameters $\theta$.


\begin{equation}
  \lambda^*(\theta) = \mbox{argmax}_{\lambda} \cL(\theta, \lambda, \cD)
\end{equation}

Both the primal and dual update steps can follow the traditional SGD training scheme \cite{fioretto2020lagrangian}.





\paragraph{Network pruning} In the scope of this paper, we focus on single shot network pruning.[CITE] This network pruning  scheme consists of the following three steps:
\begin{enumerate}
    \item \textbf{Standard training} In the first step, we perform standard training as in Equation \ref{eq:erm} to obtain optimal parameters $\theta^*$.
    
    \item \textbf{Pruning}  In the second step, we prune/remove the least important parameters/filters based on some criteria (e.g., $l_1$/$l_2$ norm based) from $\theta_*$ to obtain $\bar{\theta}$.
    
    \item \textbf{Fine-tuning} In the last step, we fine-tune the pruned parameter $\bar{\theta}$ to obtain parameter $\tilde{\theta}$
\end{enumerate}
We are interested in quantifying the disparate impact on accuracy of using the $\tilde{\theta}$ compared to the before pruning parameter $\theta_*$ to different classes. 

\fi

==> NeurIPS-22_Fair-Pruning - arixv/pruningImpact.tex <==


\section{Fairness analysis in pruning: Roadmap}
\label{sec:pruning_impact}

To gain insights on how pruning may introduce unfairness, we start with providing a useful upper bound for a group's excessive loss. Its goal is to isolate key aspects of model pruning that are responsible for the observed unfairness. The following discussion assumes the loss function $\ell(\cdot)$ to be at least twice differentiable, which is the case for common ML loss functions, such as mean squared error or cross entropy loss.
\begin{theorem}
\label{thm:taylor} 
The \emph{excessive loss} of a group $a \in \cA$ is upper bounded by\footnote{
  With a slight abuse of notation, the results refer to $\bar{\btheta}$ as the homonymous vector which is extended with $k-\bar{k}$ zeros.
}: 
\begin{align}
  R(a)  \leq 
  \left\| \bm{g}_a^{\ell} \right\|
  \times \left\|  \bar{\btheta} - \optimal{\btheta}\right\|
  + 
  \frac{1}{2} \lambda \left( \bm{H}_{a}^{\ell} \right) 
  \times 
  \left\| \bar{\btheta} - \optimal{\btheta}\right\|^2 
  + 
  \cO\left( \left\|\bar{\btheta} - \optimal{\btheta} \right\|^3 \right),
  \label{eq:thm1}
\end{align}
where 
$\bm{g}_a^\ell = \nabla_{\btheta} J( \optimal{\btheta}; D_{a})$ is the vector of gradients associated with the loss function $\ell$ evaluated at $\optimal{\btheta}$ and computed using group data $D_a$,  
$\bm{H}_{a}^{\ell} = 
\nabla^2_{\btheta} J(\optimal{\btheta}; D_{a})$ is the Hessian matrix of the loss function $\ell$, at the optimal parameters vector $\optimal{\btheta}$, computed using the group data $D_a$ (henceforth simply referred to as \emph{group hessian}), and  
$\lambda(\Sigma)$ is the maximum eigenvalue of a matrix $\Sigma$.
\end{theorem}


The bound above follows from a second order Taylor expansion of the loss function, Cauchy-Schwarz inequality, and properties of the Rayleigh quotient.

Notice that, in addition to the difference in the original and pruned parameters vectors, two key terms appear in Equation \eqref{eq:thm1}: 
{\bf (1)} The norms of the gradients $\bm{g}_a^\ell$ and {\bf (2)} the maximum eigenvalue of the Hessian matrix $\bm{H}_a^\ell$ for a group $a$. Informally, the former is associated with the groups' local optimality while the latter relates to the ability of the model to separate the groups data. 
As we will show next these components represent the main sources of unfairness due to model pruning.

The following is an important corollary of Theorem \ref{thm:taylor}. It shows that the larger the pruning, the larger will be the excessive loss for a given group.  



\begin{corollary}
\label{cor:1}
Let $\bar{k}$ and $\bar{k}'$ be the size of parameter vectors $\bar{\btheta}$ and $\bar{\btheta}'$, respectively, resulting from pruning model $f_{\optimal{\btheta}}$, where $\bar{k} < \bar{k}'$ (i.e., the former model prunes more weight than the latter one). Then, for any group $a \in \cA$, 
\begin{equation}
  \tilde{R}(a, \bar{\btheta}) \geq \tilde{R}(a, \bar{\btheta}'),
\end{equation}
where $\tilde{R}(a, \bm{\omega})$ is the excessive loss upper bound computed using pruned model parameters $\bm{\omega}$ (Eq.~\eqref{eq:thm1}).
\end{corollary}


The corollary above indicates that the excess risk for a group increases as the pruning regime increase. Building on this result, the paper illustrates next why unfairness can become more significant as the pruning regime increases.

The next sections analyze the effect of gradient norms and the Hessian to unfairness in the pruned models. The theoretical claims are supported and complemented by analytical results. These results use the UTKFace dataset \cite{zhifei2017cvpr}
for a vision task whose goal is to classify ethnicity. The experiments use a ResNet-18 architecture and the pruning counterparts remove the $P\%$  parameters with the smallest absolute values for various $P$. All reported metrics are normalized and an average of 10 repetitions. 
While the theoretical analysis focuses on the notion of disparate impacts under the lens of excessive loss, the empirical results report differences in accuracy of the resulting models. The empirical results thus reflect the setting commonly adopted when measuring accuracy parity \cite{zhao2019inherent}.


We report a glimpse of the empirical results, with the purpose of supporting the theoretical claims, and extended experiments, as well as additional descriptions of the datasets and settings, are reported in Appendix \ref{sec:additional_results}. 


==> NeurIPS-22_Fair-Pruning - arixv/relatedwork.tex <==


\subsubsection*{Related work} 
Fairness and network pruning have been long studied in isolation. 
The reader is referred to the related papers and surveys on fairness 
\citep{
barocas2017fairness,caton2020fairness,dwork2012fairness,NIPS2016_9d268236,mehrabi2021survey} and 
pruning \citep{
aghli2021combining,baykal2019sipping,blalock2020state,
Renda2020Comparing,Han2015NIPS,sehwag2019compact,Wiebke2022,zhang2018systematic} 
for a review on these areas. 

The recent interest in assessing societal values of machine learning models 
has seen an increase of studies at the intersection of different properties 
of a learning model and their effects on fairness. For example, \citet{xu2021robust}
studies the setting of adversarial robustness and show that adversarial training 
introduces unfair outcomes in term of accuracy parity \cite{zhao2019inherent}. 
\citet{zhu2021rich} show that semisupervised settings can introduce unfair outcomes 
in the resulting accuracy of the learned models. 
Finally, several authors have also shown that private training can have 
unintended disparate impacts to the resulting models' outputs \cite{NEURIPS2019_eugene,fioretto:arxiv22b,
Fioretto:NeurIPS21b,Uniyal2021DPSGDVP,Zhu:AAAI2021} 
and downstream decisions \cite{pujol:20,Tran:IJCAI21}. 

Network compression has also been shown to have a profound impact towards 
the model fairness. For example, several works observed empirically that 
network compression may amplify unfairness in different learning tasks~\cite{paganini2020prune, 
Hooker2020WhatDC, Hooker2020CharacterisingBI, Joseph2020GoingBC}.
Most of the focus has been on vision tasks and in identifying the 
set of \emph{Pruning Identified Exemplars} (PIEs), the samples that are 
impacted most under the compression scheme and conclude that PIEs belongs 
to low frequency groups (those observed at the tail of the data distribution).
\citet{Blakeney2021SimonSE} further investigate how bias could be evaluated 
and mitigated in pruned neural networks using knowledge distillation while  
\citet{hosseinilearning} observed empirically that knowledge distillation 
processes may produce unfair student models. 
The impact of network compression towards fairness has also been assessed 
in natural language tasks. For example, \citet{Du2021WhatDC} and 
\citet{xu-etal-2021-beyond} empirically measure the robustness of 
compressed large language models, while \citet{Ahia2021TheLD} look 
into how compression schemes affects data-limited regimes. Finally, 
\citet{Xu2022CanMC} investigate ways to improve fairness in generative 
language models by compressing them.  
We also note that, concurrently to this work, \citet{good:22} studied 
the relative distortion in recall for various classes. They show that pruning 
has a Matthews effect on the recall for various classes and 
% subgroups and 
propose an algorithm to attenuate such an effect.

This paper builds on this body of work and their important empirical 
observations and provides a step towards a deeper theoretical understanding 
of the fairness issues arising as a result of pruning. It derives conditions
and studies the causes of unfairness in the context of pruning as well 
as it introduces mitigating guidelines. 

==> lib.tex <==
% Please download the latest anthology.bib from
%
% http://aclweb.org/anthology/anthology.bib.gz

@inproceedings{good:22,
  title   = {Recall Distortion in Neural Network Pruning and the Undecayed Pruning Algorithm},
  author  = {Aidan Good and Jiaqi Lin and Xin Yu and Hannah Sieg and Mikey Ferguson and Shandian Zhe and Jerzy Wieczorek and Thiago Serra},
  year    = {2022},
  booktitle = {Proceedings of the International Conference on Neural Information Processing Systems ({NeurIPS})}
}

@misc{https://doi.org/10.48550/arxiv.1412.6572,
  doi = {10.48550/ARXIV.1412.6572},
  
  url = {https://arxiv.org/abs/1412.6572},
  
  author = {Goodfellow, Ian J. and Shlens, Jonathon and Szegedy, Christian},
  
  keywords = {Machine Learning (stat.ML), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Explaining and Harnessing Adversarial Examples},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}



@inproceedings{guo2019sparse,
author = {Guo, Yiwen and Zhang, Chao and Zhang, Changshui and Chen, Yurong},
title = {Sparse DNNs with Improved Adversarial Robustness},
year = {2018},
booktitle = {Proceedings of the International Conference on Neural Information Processing Systems ({NeurIPS})},
pages = {240–249}
}

@article{papernot2016transferability,
  title   = {Transferability in Machine Learning: from Phenomena to Black-Box Attacks using Adversarial Samples},
  author  = {Nicolas Papernot and Patrick McDaniel and Ian Goodfellow},
  year    = {2016},
  journal = {arXiv preprint arXiv: Arxiv-1605.07277}
}

@inproceedings{NIPS2016_9d268236,
 author = {Hardt, Moritz and Price, Eric and Price, Eric and Srebro, Nati},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {D. Lee and M. Sugiyama and U. Luxburg and I. Guyon and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Equality of Opportunity in Supervised Learning},
 url = {https://proceedings.neurips.cc/paper/2016/file/9d2682367c3935defcb1f9e247a97c0d-Paper.pdf},
 volume = {29},
 year = {2016}
}

@article{barocas2017fairness,
  title={Fairness in machine learning},
  author={Barocas, Solon and Hardt, Moritz and Narayanan, Arvind},
  journal={Nips tutorial},
  volume={1},
  pages={2},
  year={2017}
}

@inproceedings{dwork2012fairness,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  pages={214--226},
  year={2012}
}


@article{mehrabi2021survey,
  title={A survey on bias and fairness in machine learning},
  author={Mehrabi, Ninareh and Morstatter, Fred and Saxena, Nripsuta and Lerman, Kristina and Galstyan, Aram},
  journal={ACM Computing Surveys (CSUR)},
  volume={54},
  number={6},
  pages={1--35},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{caton2020fairness,
  title={Fairness in machine learning: A survey},
  author={Caton, Simon and Haas, Christian},
  journal={arXiv preprint arXiv:2010.04053},
  year={2020}
}

@inproceedings{Fioretto:NeurIPS21b,
  title={Differentially Private Empirical Risk Minimization under the Fairness Lens},
  author={Tran, Cuong and Dinh, My and Fioretto, Ferdinando},
  booktitle={Advances in Neural Information Processing Systems},
  year={2021},
}




@article{fioretto:arxiv22b,
      title={Differential Privacy and Fairness in Decisions and Learning Tasks: A Survey}, 
      author={Ferdinando Fioretto and Cuong Tran and Pascal Van Hentenryck and Keyu Zhu},
      year={2022},
      journal={CoRR},
      volume={abs/2202.08187},
      url       = {https://arxiv.org/abs/2202.08187}
}

@inproceedings{Zhu:AAAI2021, 
title={Bias and Variance of Post-processing in Differential Privacy}, 
booktitle={Proceedings of the AAAI Conference on Artificial Intelligence}, 
author={Zhu, Keyu and Van Hentenryck, Pascal and Fioretto, Ferdinando}, 
year={2021}, 
pages={11177-11184} 
}

@inproceedings{Tran:IJCAI21,
  author    = {Cuong Tran and
               Ferdinando Fioretto and
               Pascal Van Hentenryck and
               Zhiyan Yao},
  editor    = {Zhi{-}Hua Zhou},
  title     = {Decision Making with Differential Privacy under a Fairness Lens},
  booktitle = {International Joint Conference on Artificial Intelligence {(IJCAI)}},
  pages     = {560--566},
  year      = {2021},
}

@inproceedings{Tran:AAAI21,
   author    = {Cuong Tran and
               Ferdinando Fioretto and
               Pascal Van Hentenryck},
  title     = {Differentially Private and Fair Deep Learning: {A} Lagrangian Dual
               Approach},
  booktitle = {Thirty-Fifth {AAAI} Conference on Artificial Intelligence},
  pages     = {9932--9939},
  publisher = {{AAAI} Press},
  year      = {2021},
}

%% Privacy / Fairness
@inproceedings{NEURIPS2019_eugene,
  title={Differential privacy has disparate impact on model accuracy},
  author={Bagdasaryan, Eugene and Poursaeed, Omid and Shmatikov, Vitaly},
  booktitle={Advances in Neural Information Processing Systems},
  pages={15479--15488},
  year={2019}
}

@misc{https://doi.org/10.48550/arxiv.2202.08187,
  doi = {10.48550/ARXIV.2202.08187},
  
  url = {https://arxiv.org/abs/2202.08187},
  
  author = {Fioretto, Ferdinando and Tran, Cuong and Van Hentenryck, Pascal and Zhu, Keyu},
  
  keywords = {Machine Learning (cs.LG), Artificial Intelligence (cs.AI), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Differential Privacy and Fairness in Decisions and Learning Tasks: A Survey},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{zhao2019inherent,
  title={Inherent tradeoffs in learning fair representations},
  author={Zhao, Han and Gordon, Geoff},
  journal={Advances in neural information processing systems},
  volume={32},
  pages={15675--15685},
  year={2019}
}

@inproceedings{cohen2019certified,
  title={Certified adversarial robustness via randomized smoothing},
  author={Cohen, Jeremy and Rosenfeld, Elan and Kolter, Zico},
  booktitle={International Conference on Machine Learning},
  pages={1310--1320},
  year={2019},
  organization={PMLR}
}

@inproceedings{DBLP:conf/nips/TranDF21,
  author    = {Cuong Tran and
               My H. Dinh and
               Ferdinando Fioretto},
  title     = {Differentially Private Empirical Risk Minimization under the Fairness
               Lens},
  booktitle = {Advances in Neural Information Processing Systems 34},
  year      = {2021}
}


@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

@article{keskar2016large,
  title={On large-batch training for deep learning: Generalization gap and sharp minima},
  author={Keskar, Nitish Shirish and Mudigere, Dheevatsa and Nocedal, Jorge and Smelyanskiy, Mikhail and Tang, Ping Tak Peter},
  journal={arXiv preprint arXiv:1609.04836},
  year={2016}
}



@article{zhang2019gradient,
  title={Why gradient clipping accelerates training: A theoretical justification for adaptivity},
  author={Zhang, Jingzhao and He, Tianxing and Sra, Suvrit and Jadbabaie, Ali},
  journal={arXiv preprint arXiv:1905.11881},
  year={2019}
}

@article{hwang2020fairfacegan,
  title={FairfaceGAN: Fairness-aware facial image-to-image translation},
  author={Hwang, Sunhee and Park, Sungho and Kim, Dohyung and Do, Mirae and Byun, Hyeran},
  journal={arXiv preprint arXiv:2012.00282},
  year={2020}
}


@inproceedings{houben2013detection,
  title={Detection of traffic signs in real-world images: The German Traffic Sign Detection Benchmark},
  author={Houben, Sebastian and Stallkamp, Johannes and Salmen, Jan and Schlipsing, Marc and Igel, Christian},
  booktitle={The 2013 international joint conference on neural networks (IJCNN)},
  pages={1--8},
  year={2013},
  organization={Ieee}
}
@article{blalock2020state,
  title={What is the state of neural network pruning?},
  author={Blalock, Davis and Ortiz, Jose Javier Gonzalez and Frankle, Jonathan and Guttag, John},
  journal={arXiv preprint arXiv:2003.03033},
  year={2020}
}
@article{xie2021model,
  title={Model compression via pruning and knowledge distillation for person re-identification},
  author={Xie, Haonan and Jiang, Wei and Luo, Hao and Yu, Hongyan},
  journal={Journal of Ambient Intelligence and Humanized Computing},
  volume={12},
  number={2},
  pages={2149--2161},
  year={2021},
  publisher={Springer}
}

@article{frankle2018lottery,
  title={The lottery ticket hypothesis: Finding sparse, trainable neural networks},
  author={Frankle, Jonathan and Carbin, Michael},
  journal={arXiv preprint arXiv:1803.03635},
  year={2018}
}
@misc{liang2021pruning,
      title={Pruning and Quantization for Deep Neural Network Acceleration: A Survey}, 
      author={Tailin Liang and John Glossner and Lei Wang and Shaobo Shi and Xiaotong Zhang},
      year={2021},
      eprint={2101.09671},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@misc{ye2018progressive,
      title={Progressive Weight Pruning of Deep Neural Networks using ADMM}, 
      author={Shaokai Ye and Tianyun Zhang and Kaiqi Zhang and Jiayu Li and Kaidi Xu and Yunfei Yang and Fuxun Yu and Jian Tang and Makan Fardad and Sijia Liu and Xiang Chen and Xue Lin and Yanzhi Wang},
      year={2018},
      eprint={1810.07378},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{yang2019quantization,
  title={Quantization networks},
  author={Yang, Jiwei and Shen, Xu and Xing, Jun and Tian, Xinmei and Li, Houqiang and Deng, Bing and Huang, Jianqiang and Hua, Xian-sheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={7308--7316},
  year={2019}
}

@article{gou2021knowledge,
  title={Knowledge distillation: A survey},
  author={Gou, Jianping and Yu, Baosheng and Maybank, Stephen J and Tao, Dacheng},
  journal={International Journal of Computer Vision},
  volume={129},
  number={6},
  pages={1789--1819},
  year={2021},
  publisher={Springer}
}

@misc{he2015deep,
      title={Deep Residual Learning for Image Recognition}, 
      author={Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
      year={2015},
      eprint={1512.03385},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
@inproceedings{buolamwini2018gender,
  title={Gender shades: Intersectional accuracy disparities in commercial gender classification},
  author={Buolamwini, Joy and Gebru, Timnit},
  booktitle={Conference on fairness, accountability and transparency},
  pages={77--91},
  year={2018},
  organization={PMLR}
}

@article{paganini2020prune,
  title={Prune Responsibly},
  author={Paganini, Michela},
  journal={arXiv preprint arXiv:2009.09936},
  year={2020}
}



@article{augasta2013pruning,
  title={Pruning algorithms of neural networks—a comparative study},
  author={Augasta, M and Kathirvalavakumar, Thangairulappan},
  journal={Open Computer Science},
  volume={3},
  number={3},
  pages={105--115},
  year={2013},
  publisher={Versita}
}

@article{chouldechova2018frontiers,
  title={The frontiers of fairness in machine learning},
  author={Chouldechova, Alexandra and Roth, Aaron},
  journal={arXiv preprint arXiv:1810.08810},
  year={2018}
}

@inproceedings{hu2020fairnn,
  title={Fairnn-conjoint learning of fair representations for fair decisions},
  author={Hu, Tongxin and Iosifidis, Vasileios and Liao, Wentong and Zhang, Hang and Yang, Michael Ying and Ntoutsi, Eirini and Rosenhahn, Bodo},
  booktitle={International Conference on Discovery Science},
  pages={581--595},
  year={2020},
  organization={Springer}
}

@article{hosseinilearning,
  title={Learning Fair from Unfair Teachers},
  author={Hosseini, Sepidehsadat and Shabani, Mohammad Amin and Jahanara, Mohammad Mahdi and Salamatian, Bahar}
}



@article{zhu2021rich,
  title={The Rich Get Richer: Disparate Impact of Semi-Supervised Learning},
  author={Zhu, Zhaowei and Luo, Tianyi and Liu, Yang},
  journal={arXiv preprint arXiv:2110.06282},
  year={2021}
}

@misc{xu2021robust,
      title={To be Robust or to be Fair: Towards Fairness in Adversarial Training}, 
      author={Han Xu and Xiaorui Liu and Yaxin Li and Anil K. Jain and Jiliang Tang},
      year={2021},
      eprint={2010.06121},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@inproceedings{binns2018fairness,
  title={Fairness in machine learning: Lessons from political philosophy},
  author={Binns, Reuben},
  booktitle={Conference on Fairness, Accountability and Transparency},
  pages={149--159},
  year={2018},
  organization={PMLR}
}

@misc{Census-voting-rights,
  author = {Census Bureau},
    title = {Voting Rights Determination file},
    year = {2016},
    url = {\url{https://www.census. gov/programs-surveys/decennial-census/about/voting-rights/voting-rights-determination-file.html}}
}




@inproceedings{mironov2017renyi,
  title={R{\'e}nyi differential privacy},
  author={Mironov, Ilya},
  booktitle={2017 IEEE 30th Computer Security Foundations Symposium (CSF)},
  pages={263--275},
  year={2017},
  organization={IEEE}
}

@inproceedings{berthelot2019mixmatch,
  title={Mixmatch: A holistic approach to semi-supervised learning},
  author={Berthelot, David and Carlini, Nicholas and Goodfellow, Ian and Papernot, Nicolas and Oliver, Avital and Raffel, Colin A},
  booktitle={NIPS},
  pages={5049--5059},
  year={2019}
}

@misc{papernot:16,
    title={Semi-supervised Knowledge Transfer for Deep Learning from Private Training Data},
    author={Nicolas Papernot and Martín Abadi and Úlfar Erlingsson and Ian Goodfellow and Kunal Talwar},
    year={2016},
    eprint={1610.05755},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@misc{pichapati:19,
    title={AdaCliP: Adaptive Clipping for Private SGD},
    author={Venkatadheeraj Pichapati and Ananda Theertha Suresh and Felix X. Yu and Sashank J. Reddi and Sanjiv Kumar},
    year={2019},
    eprint={1908.07643},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{mcmahan:18,
    title={A General Approach to Adding Differential Privacy to Iterative Training Procedures},
    author={H. Brendan McMahan and Galen Andrew and Ulfar Erlingsson and Steve Chien and Ilya Mironov and Nicolas Papernot and Peter Kairouz},
    year={2018},
    eprint={1812.06210},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{alex2018frontiers,
    title={The Frontiers of Fairness in Machine Learning},
    author={Alexandra Chouldechova and Aaron Roth},
    year={2018},
    eprint={1810.08810},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}


%% Differential Privacy
@inproceedings{dwork:06,
  title={Calibrating noise to sensitivity in private data analysis},
  author={Dwork, Cynthia and McSherry, Frank and Nissim, Kobbi and Smith, Adam},
  booktitle={Proceedings of Theory of Cryptography Conference},
  pages={265--284},
  year={2006},
  organization={Springer}
}

@article{dwork:14,
  title={The algorithmic foundations of differential privacy},
  author={Dwork, Cynthia and Roth, Aaron and others},
  journal={Foundations and Trends{\textregistered} in Theoretical Computer Science},
  volume={9},
  number={3--4},
  pages={211--407},
  year={2014},
  publisher={Now Publishers, Inc.}
}

@article{soria:17,
  title={Individual differential privacy: A utility-preserving formulation of differential privacy guarantees},
  author={Soria-Comas, Jordi and Domingo-Ferrer, Josep and S{\'a}nchez, David and Meg{\'\i}as, David},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={12},
  number={6},
  pages={1418--1429},
  year={2017},
  publisher={IEEE}
}

% Empirical Privacy
@inproceedings{cormode:13,
  title={Empirical privacy and empirical utility of anonymized data},
  author={Cormode, Graham and Procopiuc, Cecilia M and Shen, Entong and Srivastava, Divesh and Yu, Ting},
  booktitle={2013 IEEE 29th International Conference on Data Engineering Workshops (ICDEW)},
  pages={77--82},
  year={2013},
  organization={IEEE}
}

@article{petti:19,
  title={Differential privacy in the 2020 US census: what will it do? Quantifying the accuracy/privacy tradeoff},
  author={Petti, Samantha and Flaxman, Abraham},
  journal={Gates Open Research},
  volume={3:1722},
  year={2020},
  publisher={Gates Foundation-Open Access}
}

@phdthesis{kassem:18,
  title={Differential Inference Testing A Practical Approach to Evaluate Anonymized Data},
  author={Kassem, Ali and Acs, Gergely and Castelluccia, Claude and Palamidessi, Catuscia},
  year={2018},
  school={INRIA}
}

@inproceedings{shokri:17,
  title={Membership inference attacks against machine learning models},
  author={Shokri, Reza and Stronati, Marco and Song, Congzheng and Shmatikov, Vitaly},
  booktitle={2017 IEEE Symposium on Security and Privacy (SP)},
  pages={3--18},
  year={2017},
  organization={IEEE}
}

%% Fairness 
@inproceedings{dwork:12,
  title={Fairness through awareness},
  author={Dwork, Cynthia and Hardt, Moritz and Pitassi, Toniann and Reingold, Omer and Zemel, Richard},
  booktitle={Proceedings of the 3rd innovations in theoretical computer science conference},
  year={2012}
}

@inproceedings{zafar:17,
  title={Fairness beyond disparate treatment \& disparate impact: Learning classification without disparate mistreatment},
  author={Zafar, Muhammad Bilal and Valera, Isabel and Gomez Rodriguez, Manuel and Gummadi, Krishna P},
  booktitle={Proceedings of the 26th International Conference on World Wide Web (WWW)},
  year={2017}
}

@inproceedings{feldman:15,
  title={Certifying and removing disparate impact},
  author={Feldman, Michael and Friedler, Sorelle A and Moeller, John and Scheidegger, Carlos and Venkatasubramanian, Suresh},
  booktitle={proceedings of the 21th ACM SIGKDD international conference on knowledge discovery and data mining},
  year={2015}
}



@inproceedings{hardt:16,
 author = {Hardt, Moritz and Price, Eric and Price, Eric and Srebro, Nati},
title = {Equality of Opportunity in Supervised Learning},
booktitle = {Proceedings of Advances in Neural Information Processing Systems (NIPS)},
year = {2016}
}

@inproceedings{pujol:20,
  title={Fair decision making using privacy-protected data},
  author={Pujol, David and McKenna, Ryan and Kuppam, Satya and Hay, Michael and Machanavajjhala, Ashwin and Miklau, Gerome},
  booktitle={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency (FAT) },
  pages={189--199},
  year={2020}
}

@inproceedings{agarwal:18,
  title={A Reductions Approach to Fair Classification},
  author={Agarwal, Alekh and Beygelzimer, Alina and Dudik, Miroslav and Langford, John and Wallach, Hanna},
  booktitle = {Proceedings of the International Conference on Machine Learning ({ICML})},
  year={2018}
}

@inproceedings{fioretto2020lagrangian,
      title={Lagrangian Duality for Constrained Deep Learning}, 
      author={Ferdinando Fioretto and Pascal {Van Hentenryck} and {Terrence WK} Mak and Cuong Tran and Federico Baldo and Michele Lombardi},
      pages={118--135},
      year={2020},
      booktitle="European Conference on Machine Learning and Principles and Practice of Knowledge Discovery in Databases ({ECML-PKDD})"
}


@misc{Fioretto:ArXiv20b,
    title="A Lagrangian Dual Framework for Deep Neural Networks with Constraints Optimization",
    author="Ferdinando Fioretto and Terrence {W.K. Mak} and 
     Federico Baldo and Michele Lombardi and  Pascal {Van Hentenryck}",
    year="2020",
    eprint="2001.09394",
    archivePrefix="arXiv",
    primaryClass="cs.LG",
    secondaryClass="stat.ML"
}

@article{Fioretto:AAAI20, 
    title={Predicting AC Optimal Power Flows: Combining Deep Learning and Lagrangian Dual Methods}, 
    volume={34}, 
    number={01}, 
    journal={Proceedings of the AAAI Conference on Artificial Intelligence}, 
    author={Fioretto, Ferdinando and Mak, {Terrence W.K.} and {Van Hentenryck}, Pascal}, 
    year={2020}, 
    pages={630-637} 
}


%% Fairness and Privacy
@inproceedings{cummings:19,
  title={On the compatibility of privacy and fairness},
  author={Cummings, Rachel and Gupta, Varun and Kimpara, Dhamma and Morgenstern, Jamie},
  booktitle={Proceedings of the Adjunct Publication of the 27th Conference on User Modeling, Adaptation and Personalization (UMAP)},
  year={2019}
}

@article{dwork35s,
  title={It’s Not Privacy and It’s Not Fair, 66 Stan},
  author={Dwork, Cynthia and Mulligan, Deirdre K},
  journal={L. Rev. Online},
  volume={35}
}

@inproceedings{ekstrand:18,
  title={Privacy for all: Ensuring fair and equitable privacy protections},
  author={Ekstrand, Michael D and Joshaghani, Rezvan and Mehrpouyan, Hoda},
  booktitle={Proceedings of  Conference on Fairness, Accountability and Transparency},
  pages={35--47},
  year={2018}
}

%% Constrained Learning
@InProceedings{Fontaine:14,
  author="Fontaine, Daniel and Laurent, Michel and {Van Hentenryck}, Pascal",
  title="Constraint-Based Lagrangian Relaxation",
  booktitle="Principles and Practice of Constraint Programming",
  year="2014",
  pages="324--339",
}



@article{Hestenes:69,
  title={Multiplier and gradient methods},
  author={Hestenes, Magnus R},
  journal={Journal of optimization theory and applications},
  volume={4},
  number={5},
  pages={303--320},
  year={1969},
  publisher={Springer}
}

@article{boyd2011distributed,
  title={Distributed optimization and statistical learning via the alternating direction method of multipliers},
  author={Boyd, Stephen and Parikh, Neal and Chu, Eric and Peleato, Borja and Eckstein, Jonathan and others},
  journal={Foundations and Trends{\textregistered} in Machine learning},
  volume={3},
  number={1},
  pages={1--122},
  year={2011},
  publisher={Now Publishers, Inc.}
}


%% Privacy / Fairness
@inproceedings{bagdasaryan:19,
  title={Differential privacy has disparate impact on model accuracy},
  author={Bagdasaryan, Eugene and Poursaeed, Omid and Shmatikov, Vitaly},
  booktitle={Proceedings of Advances in Neural Information Processing Systems (NIPS)},
  year={2019}
}

@inproceedings{goodman2016step,
  title={A step towards accountable algorithms? algorithmic discrimination and the european union general data protection},
  author={Goodman, Bryce W},
  booktitle={29th Conference on Neural Information Processing Systems (NIPS 2016), Barcelona. NIPS Foundation},
  year={2016}
}

@article{DBLP:journals/corr/SmithCST17,
  author    = {Virginia Smith and
               Chao{-}Kai Chiang and
               Maziar Sanjabi and
               Ameet Talwalkar},
  title     = {Federated Multi-Task Learning},
  journal   = {CoRR},
  volume    = {abs/1705.10467},
  year      = {2017},
  url       = {http://arxiv.org/abs/1705.10467}
}

@inproceedings{zafar2015fairness,
title={Fairness Constraints: Mechanisms for Fair Classification},
author={Muhammad Bilal Zafar and Isabel Valera and Manuel Gomez Rodriguez and Krishna P. Gummadi},
booktitle={Proceedings of Artificial Intelligence and Statistics (AISTAT)},
year={2017}
}

@inproceedings{chidlovskii2016domain,
  title={Domain adaptation in the absence of source domain data},
  author={Chidlovskii, Boris and Clinchant, St{\'e}phane and Csurka, Gabriela},
  booktitle={Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={451--460},
  year={2016},
  organization={ACM}
}

@inproceedings{xu2019achieving,
  title={Achieving Differential Privacy and Fairness in Logistic Regression},
  author={Xu, Depeng and Yuan, Shuhan and Wu, Xintao},
  booktitle={Proceedings of the 26th International Conference on World Wide Web (WWW) },
  year={2019}
}



@inproceedings{perez2017fair,
  title={Fair kernel learning},
  author={P{\'e}rez-Suay, Adri{\'a}n and Laparra, Valero and Mateo-Garc{\'\i}a, Gonzalo and Mu{\~n}oz-Mar{\'\i}, Jordi and G{\'o}mez-Chova, Luis and Camps-Valls, Gustau},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={339--355},
  year={2017},
  organization={Springer}
}

@inproceedings{kamishima2012fairness,
  title={Fairness-aware classifier with prejudice remover regularizer},
  author={Kamishima, Toshihiro and Akaho, Shotaro and Asoh, Hideki and Sakuma, Jun},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={35--50},
  year={2012},
  organization={Springer}
}

@misc{li2019fair,
    title={Fair Resource Allocation in Federated Learning},
    author={Tian Li and Maziar Sanjabi and Virginia Smith},
    year={2019},
    eprint={1905.10497},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{liang2020think,
    title={Think Locally, Act Globally: Federated Learning with Local and Global Representations},
    author={Paul Pu Liang and Terrance Liu and Liu Ziyin and Ruslan Salakhutdinov and Louis-Philippe Morency},
    year={2020},
    eprint={2001.01523},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{kairouz2019advances,
    title={Advances and Open Problems in Federated Learning},
    author={Peter Kairouz and H. Brendan McMahan and Brendan Avent and Aurélien Bellet and Mehdi Bennis and Arjun Nitin Bhagoji and Keith Bonawitz and Zachary Charles and Graham Cormode and Rachel Cummings and Rafael G. L. D'Oliveira and Salim El Rouayheb and David Evans and Josh Gardner and Zachary Garrett and Adrià Gascón and Badih Ghazi and Phillip B. Gibbons and Marco Gruteser and Zaid Harchaoui and Chaoyang He and Lie He and Zhouyuan Huo and Ben Hutchinson and Justin Hsu and Martin Jaggi and Tara Javidi and Gauri Joshi and Mikhail Khodak and Jakub Konečný and Aleksandra Korolova and Farinaz Koushanfar and Sanmi Koyejo and Tancrède Lepoint and Yang Liu and Prateek Mittal and Mehryar Mohri and Richard Nock and Ayfer Özgür and Rasmus Pagh and Mariana Raykova and Hang Qi and Daniel Ramage and Ramesh Raskar and Dawn Song and Weikang Song and Sebastian U. Stich and Ziteng Sun and Ananda Theertha Suresh and Florian Tramèr and Praneeth Vepakomma and Jianyu Wang and Li Xiong and Zheng Xu and Qiang Yang and Felix X. Yu and Han Yu and Sen Zhao},
    year={2019},
    eprint={1912.04977},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}


@incollection{NIPS2017_6670,
title = {Recycling Privileged Learning and Distribution Matching for Fairness},
author = {Quadrianto, Novi and Sharmanska, Viktoriia},
booktitle = {NIPS},
year = {2017}
}

@misc{woodworth2017learning,
    title={Learning Non-Discriminatory Predictors},
    author={Blake Woodworth and Suriya Gunasekar and Mesrob I. Ohannessian and Nathan Srebro},
    year={2017},
    eprint={1702.06081},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}


@misc{mehrabi2019survey,
    title={A Survey on Bias and Fairness in Machine Learning},
    author={Ninareh Mehrabi and Fred Morstatter and Nripsuta Saxena and Kristina Lerman and Aram Galstyan},
    year={2019},
    eprint={1908.09635},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{article,
author = {Adel, Tameem and Valera, Isabel and Ghahramani, Zoubin and Weller, Adrian},
year = {2019},
month = {07},
pages = {2412-2420},
title = {One-Network Adversarial Fairness},
volume = {33},
journal = {Proceedings of the AAAI Conference on Artificial Intelligence},
doi = {10.1609/aaai.v33i01.33012412}
}


@article{DBLP:journals/corr/abs-1805-11202,
  author    = {Depeng Xu and
               Shuhan Yuan and
               Lu Zhang and
               Xintao Wu},
  title     = {FairGAN: Fairness-aware Generative Adversarial Networks},
  journal   = {CoRR},
  volume    = {abs/1805.11202},
  year      = {2018},
  url       = {http://arxiv.org/abs/1805.11202},
  archivePrefix = {arXiv},
  eprint    = {1805.11202}
}

@incollection{zhao2019conditional,
    title={Conditional Learning of Fair Representations},
    author={Han Zhao and Amanda Coston and Tameem Adel and Geoffrey J. Gordon},
    booktitle = {ICLR},
    year={2019}
}

@article{DBLP:journals/corr/abs-1910-07162,
  author    = {Han Zhao and
               Amanda Coston and
               Tameem Adel and
               Geoffrey J. Gordon},
  title     = {Conditional Learning of Fair Representations},
  journal   = {CoRR},
  volume    = {abs/1910.07162},
  year      = {2019},
  url       = {http://arxiv.org/abs/1910.07162},
  archivePrefix = {arXiv},
  eprint    = {1910.07162},
  timestamp = {Tue, 22 Oct 2019 18:17:16 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1910-07162.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@incollection{NIPS2017_6699,
title = {Learning to Pivot with Adversarial Networks},
author = {Louppe, Gilles and Kagan, Michael and Cranmer, Kyle},
booktitle = {Advances in Neural Information Processing Systems 30},
year = {2017}
}

@incollection{NIPS2016_6374,
title = {Equality of Opportunity in Supervised Learning},
author = {Hardt, Moritz and Price, Eric and Price, Eric and Srebro, Nati},
booktitle = {NIPS},
year = {2016}
}

@inproceedings{DBLP:conf/icdm/CaldersKKAZ13,
 author    = {Toon Calders and
               Asim Karim and
               Faisal Kamiran and
               Wasif Ali and
               Xiangliang Zhang},
  title     = {Controlling Attribute Effect in Linear Regression},
  booktitle = {ICDM},
  year      = {2013}
}

@misc{edwards2015censoring,
    title={Censoring Representations with an Adversary},
    author={Harrison Edwards and Amos Storkey},
    year={2015},
    eprint={1511.05897},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@misc{beutel2017data,
    title={Data Decisions and Theoretical Implications when Adversarially Learning Fair Representations},
    author={Alex Beutel and Jilin Chen and Zhe Zhao and Ed H. Chi},
    year={2017},
    eprint={1707.00075},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@incollection{NIPS2017_7151,
title = {On Fairness and Calibration},
author = {Pleiss, Geoff and Raghavan, Manish and Wu, Felix and Kleinberg, Jon and Weinberger, Kilian Q},
booktitle = {Advances in Neural Information Processing Systems 30},
year = {2017}
}

@inproceedings{10.5555/3327144.3327203,
author = {Donini, Michele and Oneto, Luca and Ben-David, Shai and Shawe-Taylor, John and Pontil, Massimiliano},
title = {Empirical Risk Minimization under Fairness Constraints},
year = {2018},
booktitle = {NIPS}
}


@inproceedings{Feldman2015ComputationalFP,
  title={Computational Fairness: Preventing Machine-Learned Discrimination},
  author={Michael Feldman},
  year={2015}
}

@article{DBLP:journals/corr/abs-1812-06135,
  author    = {Pranay Kr. Lohia and
               Karthikeyan Natesan Ramamurthy and
               Manish Bhide and
               Diptikalyan Saha and
               Kush R. Varshney and
               Ruchir Puri},
  title     = {Bias Mitigation Post-processing for Individual and Group Fairness},
  journal   = {CoRR},
  volume    = {abs/1812.06135},
  year      = {2018},
  url       = {http://arxiv.org/abs/1812.06135},
  archivePrefix = {arXiv},
  eprint    = {1812.06135},
  timestamp = {Tue, 01 Jan 2019 15:01:25 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1812-06135.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{10.1145/3306618.3314287,
author = {Kim, Michael P. and Ghorbani, Amirata and Zou, James},
title = {Multiaccuracy: Black-Box Post-Processing for Fairness in Classification},
year = {2019},
booktitle = {Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society}
}
  
@inproceedings{10.5555/3045118.3045244,
author = {Ganin, Yaroslav and Lempitsky, Victor},
title = {Unsupervised Domain Adaptation by Backpropagation},
year = {2015},
publisher = {JMLR.org},
booktitle = {Proceedings of the 32nd International Conference on International Conference on Machine Learning - Volume 37},
pages = {1180–1189},
numpages = {10},
location = {Lille, France},
series = {ICML’15}
}
    
@incollection{NIPS2014_5423,
title = {Generative Adversarial Nets},
author = {Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems 27},
editor = {Z. Ghahramani and M. Welling and C. Cortes and N. D. Lawrence and K. Q. Weinberger},
pages = {2672--2680},
year = {2014},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/5423-generative-adversarial-nets.pdf}
}

@inproceedings{10.1145/3306618.3314255,
author = {Oneto, Luca and Doninini, Michele and Elders, Amon and Pontil, Massimiliano},
title = {Taking Advantage of Multitask Learning for Fair Classification},
year = {2019},
booktitle = {Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society}
}

@incollection{NIPS2017_6699,
title = {Learning to Pivot with Adversarial Networks},
author = {Louppe, Gilles and Kagan, Michael and Cranmer, Kyle},
booktitle = {Advances in Neural Information Processing Systems 30},
editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
pages = {981--990},
year = {2017},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/6699-learning-to-pivot-with-adversarial-networks.pdf}
}

@article{DBLP:journals/corr/ShokriSS16,
  author    = {Reza Shokri and
               Marco Stronati and
               Vitaly Shmatikov},
  title     = {Membership Inference Attacks against Machine Learning Models},
  journal   = {CoRR},
  volume    = {abs/1610.05820},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.05820},
  archivePrefix = {arXiv},
  eprint    = {1610.05820},
  timestamp = {Mon, 13 Aug 2018 16:47:19 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ShokriSS16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}




@article{10.1561/0400000042,
author = {Dwork, Cynthia and Roth, Aaron},
title = {The Algorithmic Foundations of Differential Privacy},
year = {2014},
issue_date = {August 2014},
publisher = {Now Publishers Inc.},
journal = {Found. Trends Theor. Comput. Sci.},
month = aug,
pages = {211–407},
numpages = {197}
}

@article{Black_2020,
   title={FlipTest},
   ISBN={9781450369367},
   url={http://dx.doi.org/10.1145/3351095.3372845},
   DOI={10.1145/3351095.3372845},
   journal={Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
   publisher={ACM},
   author={Black, Emily and Yeom, Samuel and Fredrikson, Matt},
   year={2020},
   month={Jan}
}
@misc{cotter2018twoplayer,
    title={Two-Player Games for Efficient Non-Convex Constrained Optimization},
    author={Andrew Cotter and Heinrich Jiang and Karthik Sridharan},
    year={2018},
    eprint={1804.06500},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@incollection{NIPS2019_8322,
title = {Noise-tolerant fair classification},
author = {Lamy, Alex and Zhong, Ziyuan and Menon, Aditya K and Verma, Nakul},
booktitle = {NIPS},
year = {2019},
}


@InProceedings{Jagielski:20,
  title = 	 {Differentially Private Fair Learning},
  author = 	 {Jagielski, Matthew and Kearns, Michael and Mao, Jieming and Oprea, Alina and Roth, Aaron and -Malvajerdi, Saeed Sharifi and Ullman, Jonathan},
  booktitle = 	 {Proceedings of the 36th International Conference on Machine Learning (ICML)},
  year = 	 {2019}
}

@misc{eban2016scalable,
    title={Scalable Learning of Non-Decomposable Objectives},
    author={Elad ET. Eban and Mariano Schain and Alan Mackey and Ariel Gordon and Rif A. Saurous and Gal Elidan},
    year={2016},
    eprint={1608.04802},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}


@InProceedings{pmlr-v98-cotter19a,
  title = 	 {Two-Player Games for Efficient Non-Convex Constrained Optimization},
  author = 	 {Cotter, Andrew and Jiang, Heinrich and Sridharan, Karthik},
  booktitle = 	 {Proceedings of the 30th International Conference on Algorithmic Learning Theory},
  year = 	 {2019},
  series = 	 {Proceedings of Machine Learning Research},}
}

@misc{cotter2018optimization,
    title={Optimization with Non-Differentiable Constraints with Applications to Fairness, Recall, Churn, and Other Goals},
    author={Andrew Cotter and Heinrich Jiang and Serena Wang and Taman Narayan and Maya Gupta and Seungil You and Karthik Sridharan},
    year={2018},
    archivePrefix={arXiv},
}


@misc{wang2020robust,
    title={Robust Optimization for Fairness with Noisy Protected Groups},
    author={Serena Wang and Wenshuo Guo and Harikrishna Narasimhan and Andrew Cotter and Maya Gupta and Michael I. Jordan},
    year={2020},
    archivePrefix={arXiv}
}

@misc{awasthi2019equalized,
    title={Equalized odds postprocessing under imperfect group information},
    author={Pranjal Awasthi and Matthäus Kleindessner and Jamie Morgenstern},
    year={2019},
    booktitle ={arXiv},
    primaryClass={stat.ML}
}

@InProceedings{pmlr-v80-kilbertus18a,
  title = 	 {Blind Justice: Fairness with Encrypted Sensitive Attributes},
  author = 	 {Kilbertus, Niki and Gascon, Adria and Kusner, Matt and Veale, Michael and Gummadi, Krishna and Weller, Adrian},
  year = 	 {2018},
  series = 	 {Proceedings of Machine Learning Research},
}

@misc{alabi2019cost,
    title={The Cost of a Reductions Approach to Private Fair Optimization},
    author={Daniel Alabi},
    year={2019},
    archivePrefix={arXiv},
}


@InProceedings{mozannar2020fair,
  title = 	 {Fair Learning with Private Demographic Data},
  author = 	 {Hussein Mozannar and Mesrob I. Ohannessian and Nathan Srebro},
 booktitle = {Proceedings of the International Conference on Machine Learning (ICML)},
  year = {2020}
}

@incollection{NIPS2014_5392,
title = {Extremal Mechanisms for Local Differential Privacy},
author = {Kairouz, Peter and Oh, Sewoong and Viswanath, Pramod},
booktitle = {Proceedings of Advances in Neural Information Processing Systems (NIPS)},
year = {2014}
}




@inproceedings{abadi:16,
author = {Abadi, Martin and Chu, Andy and Goodfellow, Ian and McMahan, H. Brendan and Mironov, Ilya and Talwar, Kunal and Zhang, Li},
title = {Deep Learning with Differential Privacy},
year = {2016},
booktitle = {Proceedings of the 2016 ACM SIGSAC Conference on Computer and Communications Security}
}


@misc{kuppam2019fair,
    title={Fair Decision Making using Privacy-Protected Data},
    author={Satya Kuppam and Ryan Mckenna and David Pujol and Michael Hay and Ashwin Machanavajjhala and Gerome Miklau},
    year={2019},
    archivePrefix={arXiv}
}


@article{JMLR:v12:chaudhuri11a,
  author  = {Kamalika Chaudhuri and Claire Monteleoni and Anand D. Sarwate},
  title   = {Differentially Private Empirical Risk Minimization},
  journal = {Journal of Machine Learning Research},
  year    = {2011},
}

@misc{shokri2016membership,
    title={Membership Inference Attacks against Machine Learning Models},
    author={Reza Shokri and Marco Stronati and Congzheng Song and Vitaly Shmatikov},
    year={2016},
    eprint={1610.05820},
    archivePrefix={arXiv},
    primaryClass={cs.CR}
}

@misc{ferdin2020lagrangian,
    title={Lagrangian Duality for Constrained Deep Learning},
    author={Ferdinando Fioretto and Pascal Van Hentenryck and Terrence WK Mak and Cuong Tran and Federico Baldo and Michele Lombardi},
    year={2020},
    eprint={2001.09394},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@InProceedings{pmlr-v97-amin19a,
  title = 	 {Bounding User Contributions: A Bias-Variance Trade-off in Differential Privacy},
  author = 	 {Amin, Kareem and Kulesza, Alex and Munoz, Andres and Vassilvtiskii, Sergei},
  booktitle = 	 {ICML},
  year = 	 {2019},
}

@article{acs2018differentially,
  title={Differentially private mixture of generative neural networks},
  author={Acs, Gergely and Melis, Luca and Castelluccia, Claude and De Cristofaro, Emiliano},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  year={2018},
}







@article{xie2018differentially,
  title={Differentially private generative adversarial network},
  author={Xie, Liyang and Lin, Kaixiang and Wang, Shu and Wang, Fei and Zhou, Jiayu},
  journal={arXiv preprint arXiv:1802.06739},
  year={2018}
}

@article{Tran2020DifferentiallyPA,
  title={Differentially Private and Fair Deep Learning: A Lagrangian Dual Approach},
  author={Cuong Tran and Ferdinando Fioretto and Pascal {Van Hentenryck}},
  journal={ArXiv},
  year={2020},
  volume={abs/2009.12562}
}



@article{mironov2019r,
  title={R$\backslash$'enyi Differential Privacy of the Sampled Gaussian Mechanism},
  author={Mironov, Ilya and Talwar, Kunal and Zhang, Li},
  journal={ArXiv},
  year={2019},
  volume={abs/1908.10530}
}

@article{subramani2020enabling,
      title={Enabling Fast Differentially Private SGD via Just-in-Time Compilation and Vectorization}, 
      author={Pranav Subramani and Nicholas Vadivelu and Gautam Kamath},
        journal={ArXiv},
      year={2020},
     volume={abs/2010.09063}
}


@INPROCEEDINGS{Han2015NIPS,
  author={S. Han, J. Pool, J. Tran and W. J. Dally},
  booktitle={NIPS}, 
  title={Learning both weights and connections for efficient neural networks}, 
  year={2015},
  volume={},
  number={},
  url = {https://arxiv.org/abs/1506.02626v3},
}

@inproceedings{wu2016quantized,
  title={Quantized convolutional neural networks for mobile devices},
  author={Wu, Jiaxiang and Leng, Cong and Wang, Yuhang and Hu, Qinghao and Cheng, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4820--4828},
  year={2016}
}

@inproceedings{NIPS1988_07e1cd7d,
author = {Mozer, Michael C and Smolensky, Paul},
booktitle = {Advances in Neural Information Processing Systems},
editor = {D. Touretzky},
pages = {},
publisher = {Morgan-Kaufmann},
title = {Skeletonization: A Technique for Trimming the Fat from a Network via Relevance Assessment},
url = {https://proceedings.neurips.cc/paper/1988/file/07e1cd7dca89a1678042477183b7ac3f-Paper.pdf},
volume = {1},
year = {1988}
}


@inproceedings{
Renda2020Comparing,
title={Comparing Rewinding and Fine-tuning in Neural Network Pruning},
author={Alex Renda and Jonathan Frankle and Michael Carbin},
booktitle={International Conference on Learning Representations},
year={2020},
url={https://openreview.net/forum?id=S1gSj0NKvB}
}


@article{baykal2019sipping,
  title={Sipping neural networks: Sensitivity-informed provable pruning of neural networks},
  author={Baykal, Cenk and Liebenwein, Lucas and Gilitschenski, Igor and Feldman, Dan and Rus, Daniela},
  journal={arXiv preprint arXiv:1910.05422},
  year={2019}
}


@article{hinton2015distilling,
  title={Distilling the knowledge in a neural network},
  author={Hinton, Geoffrey and Vinyals, Oriol and Dean, Jeff and others},
  journal={arXiv preprint arXiv:1503.02531},
  volume={2},
  number={7},
  year={2015}
}

@inproceedings{zhang2018systematic,
  title={A systematic dnn weight pruning framework using alternating direction method of multipliers},
  author={Zhang, Tianyun and Ye, Shaokai and Zhang, Kaiqi and Tang, Jian and Wen, Wujie and Fardad, Makan and Wang, Yanzhi},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={184--199},
  year={2018}
}



@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}



@inproceedings{luo2017thinet,
  title={Thinet: A filter level pruning method for deep neural network compression},
  author={Luo, Jian-Hao and Wu, Jianxin and Lin, Weiyao},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5058--5066},
  year={2017}
}


@article{sehwag2019compact,
      title={Towards Compact and Robust Deep Neural Networks}, 
      Author={Sehwag,Vikash  and Wang, Shiqi  and Mittal, Prateek  and Jana,Suman },
      year={2019},
      eprint={1906.06110},
      journal={preprint arXiv:1906.06110},
      primaryClass={cs.LG}
}

@inproceedings{aghli2021combining,
  title={Combining Weight Pruning and Knowledge Distillation for CNN Compression},
  author={Aghli, Nima and Ribeiro, Eraldo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={3191--3198},
  year={2021}
}
@article{prakosa2021improving,
  title={Improving the accuracy of pruned network using knowledge distillation},
  author={Prakosa, Setya Widyawan and Leu, Jenq-Shiou and Chen, Zhao-Hong},
  journal={Pattern Analysis and Applications},
  volume={24},
  number={2},
  pages={819--830},
  year={2021},
  publisher={Springer}
}

@inproceedings{zhu2017prune,
  author    = {Michael Zhu and
               Suyog Gupta},
  title     = {To Prune, or Not to Prune: Exploring the Efficacy of Pruning for Model
               Compression},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
               Vancouver, BC, Canada, April 30 - May 3, 2018, Workshop Track Proceedings},
  publisher = {OpenReview.net},
  year      = {2018},
  url       = {https://openreview.net/forum?id=Sy1iIDkPM},
  timestamp = {Thu, 04 Apr 2019 13:20:09 +0200},
  biburl    = {https://dblp.org/rec/conf/iclr/ZhuG18.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{li2016pruning,
  title={Pruning filters for efficient convnets},
  author={Li, Hao and Kadav, Asim and Durdanovic, Igor and Samet, Hanan and Graf, Hans Peter},
  booktitle={Proceedings of the 5th International Conference on Learning Representations (ICLR’17)},
  year={2017}
}

@article{cifar10,
title= {CIFAR-10 (Canadian Institute for Advanced Research)},
journal= {},
author= {Alex Krizhevsky and Vinod Nair and Geoffrey Hinton},
year= {},
url= {http://www.cs.toronto.edu/~kriz/cifar.html},
abstract= {The CIFAR-10 dataset consists of 60000 32x32 colour images in 10 classes, with 6000 images per class. There are 50000 training images and 10000 test images. 

The dataset is divided into five training batches and one test batch, each with 10000 images. The test batch contains exactly 1000 randomly-selected images from each class. The training batches contain the remaining images in random order, but some training batches may contain more images from one class than another. Between them, the training batches contain exactly 5000 images from each class. },
keywords= {Dataset},
terms= {}
}


@inproceedings{he2017channel,
  title={Channel pruning for accelerating very deep neural networks},
  author={He, Yihui and Zhang, Xiangyu and Sun, Jian},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={1389--1397},
  year={2017}
}


@inproceedings{
liu2018rethinking,
title={Rethinking the Value of Network Pruning},
author={Zhuang Liu and Mingjie Sun and Tinghui Zhou and Gao Huang and Trevor Darrell},
booktitle={International Conference on Learning Representations},
year={2019},
}

@inproceedings{Netzer2011ReadingDI,
  title={Reading Digits in Natural Images with Unsupervised Feature Learning},
  author={Yuval Netzer and Tao Wang and Adam Coates and A. Bissacco and Bo Wu and A. Ng},
  year={2011}
}

@inproceedings{zhifei2017cvpr,
  title={Age Progression/Regression by Conditional Adversarial Autoencoder},
  author={Zhang, Zhifei and Song, Yang and Qi, Hairong},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  year={2017},
  organization={IEEE}
}

@inproceedings{liu2015faceattributes,
  title = {Deep Learning Face Attributes in the Wild},
  author = {Liu, Ziwei and Luo, Ping and Wang, Xiaogang and Tang, Xiaoou},
  booktitle = {Proceedings of International Conference on Computer Vision (ICCV)},
  month = {December},
  year = {2015} 
}

@MISC{JigsawURL,
howpublished={\url{https://www.kaggle.com/c/jigsaw-unintended-bias-in-toxicity-classification}}
}

@article{paszke2017automatic,
  title={Automatic differentiation in PyTorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  year={2017}
}

@article{Uniyal2021DPSGDVP,
  title={DP-SGD vs PATE: Which Has Less Disparate Impact on Model Accuracy?},
  author={Archit Uniyal and Rakshit Naidu and Sasikanth Kotti and Sahib Singh and Patrik Joslin Kenfack and FatemehSadat Mireshghallah and Andrew Trask},
  journal={ArXiv},
  year={2021},
  volume={abs/2106.12576}
}

@article{Hooker2020WhatDC,
  title={What Do Compressed Deep Neural Networks Forget},
  author={Sara Hooker and Aaron C. Courville and Gregory Clark and Yann Dauphin and Andrea Frome},
  journal={arXiv: Learning},
  year={2020}
}


@article{Hooker2020CharacterisingBI,
  title={Characterising Bias in Compressed Models},
  author={Sara Hooker and Nyalleng Moorosi and Gregory Clark and Samy Bengio and Emily L. Denton},
  journal={ArXiv},
  year={2020},
  volume={abs/2010.03058}
}

@inproceedings{Joseph2020GoingBC,
  title={Going Beyond Classification Accuracy Metrics in Model Compression},
  author={Vinu Joseph and Shoaib Ahmed Siddiqui and Aditya Bhaskara and Ganesh Gopalakrishnan and Saurav Muralidharan and Michael Garland and Sheraz Ahmed and Andreas R. Dengel},
  year={2020}
}


@article{Blakeney2021SimonSE,
  title={Simon Says: Evaluating and Mitigating Bias in Pruned Neural Networks with Knowledge Distillation},
  author={Cody Blakeney and Nathaniel Huish and Yan Yan and Ziliang Zong},
  journal={ArXiv},
  year={2021},
  volume={abs/2106.07849}
}

@article{Du2021WhatDC,
  title={What do Compressed Large Language Models Forget? Robustness Challenges in Model Compression},
  author={Mengnan Du and Subhabrata Mukherjee and Yu Cheng and Milad Shokouhi and Xia Hu and Ahmed Hassan Awadallah},
  journal={ArXiv},
  year={2021},
  volume={abs/2110.08419}
}

@inproceedings{xu-etal-2021-beyond,
    title = "Beyond Preserved Accuracy: Evaluating Loyalty and Robustness of {BERT} Compression",
    author = "Xu, Canwen  and
      Zhou, Wangchunshu  and
      Ge, Tao  and
      Xu, Ke  and
      McAuley, Julian  and
      Wei, Furu",
    booktitle = "Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2021",
    address = "Online and Punta Cana, Dominican Republic",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.emnlp-main.832",
    doi = "10.18653/v1/2021.emnlp-main.832",
    pages = "10653--10659",
    abstract = "Recent studies on compression of pretrained language models (e.g., BERT) usually use preserved accuracy as the metric for evaluation. In this paper, we propose two new metrics, label loyalty and probability loyalty that measure how closely a compressed model (i.e., student) mimics the original model (i.e., teacher). We also explore the effect of compression with regard to robustness under adversarial attacks. We benchmark quantization, pruning, knowledge distillation and progressive module replacing with loyalty and robustness. By combining multiple compression techniques, we provide a practical strategy to achieve better accuracy, loyalty and robustness.",
}

@inproceedings{Ahia2021TheLD,
  title={The Low-Resource Double Bind: An Empirical Study of Pruning for Low-Resource Machine Translation},
  author={Orevaoghene Ahia and Julia Kreutzer and Sara Hooker},
  booktitle={EMNLP},
  year={2021}
}

@article{Xu2022CanMC,
  title={Can Model Compression Improve NLP Fairness},
  author={Guangxuan Xu and Qingyuan Hu},
  journal={ArXiv},
  year={2022},
  volume={abs/2201.08542}
}


@article{Stoychev2022TheEO,
  title={The Effect of Model Compression on Fairness in Facial Expression Recognition},
  author={Samuil Stoychev and Hatice Gunes},
  journal={ArXiv},
  year={2022},
  volume={abs/2201.01709}
}

@misc{Wiebke2022,
  doi = {10.48550/ARXIV.2201.07677},
  
  url = {https://arxiv.org/abs/2201.07677},
  
  author = {Toussaint, Wiebke and Mathur, Akhil and Kawsar, Fahim and Ding, Aaron Yi},
  
  keywords = {Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Tiny, always-on and fragile: Bias propagation through design choices in on-device machine learning workflows},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

